Rainier: Reinforced Knowledge Introspector for Commonsense Question Answering

Knowledge underpins reasoning. Recent research demonstrates that when relevant knowledge is provided as additional context to commonsense question answering (QA), it can substantially enhance the performance even on top of state-of-the-art. The fundamental challenge is where and how to find such knowledge that is high quality and on point with respect to the question; knowledge retrieved from knowledge bases are incomplete and knowledge generated from language models are inconsistent. We present Rainier, or Reinforced Knowledge Introspector, that learns to generate contextually relevant knowledge in response to given questions. Our approach starts by imitating knowledge generated by GPT-3, then learns to generate its own knowledge via reinforcement learning where rewards are shaped based on the increased performance on the resulting question answering. Rainier demonstrates substantial and consistent performance gains when tested over 9 different commonsense benchmarks: including 5 datasets that are seen during model training, as well as 4 datasets that are kept unseen. Our work is the first to report that knowledge generated by models that are orders of magnitude smaller than GPT-3, even without direct supervision on the knowledge itself, can exceed the quality of commonsense knowledge elicited from GPT-3.

==> [EMNLP 2022] cc-GKM/floats/ablations.tex <==
\begin{table*}[t]
\begin{minipage}[t]{.30 \linewidth}
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{1.0 \textwidth}{!}{%
\begin{tabular}{l cc}
\toprule
\textbf{QA Model} $\rightarrow$ & \multicolumn{2}{c}{UQA-large} \\
\textbf{Knowledge Gen.} $\downarrow$ & seen & unseen \\
\midrule
None & 55.07 & 39.59 \\
\midrule
\methodname{}-large & \textbf{60.36} & \textbf{41.53} \\
\quad -- Stage I & 53.68 & 36.83 \\
\quad -- Stage II & 57.00 & 40.70 \\
\quad -- Stage I -- Stage II & 53.29 & 36.72 \\
\bottomrule
\end{tabular}
}%
\vspace{-4pt}
\caption{
    Ablations on the importance of both training stages.
}
\label{tab:ablation_stages}
\end{minipage}
\hfill
\begin{minipage}[t]{.68 \linewidth}
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{1.0 \textwidth}{!}{%
\begin{tabular}{ll cc}
\toprule
\textbf{QA Model} $\rightarrow$ &  & \multicolumn{2}{c}{UQA-large} \\
\textbf{Reward Func.} $\downarrow$ & \textbf{Definition:} $r(x, k) = \hdots$ & seen & unseen \\
\midrule
\methodname{}'s & $\frac{1}{2} \Big[ \tanh \big( \Sqa{a^* | q \circ k} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q \circ k} \big)$ \\ & $\qquad - \tanh \big( \Sqa{a^* | q} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q} \big) \Big]$ & 60.36 & \textbf{41.53} \\
\midrule
Prob only & $\Pqa{a^* | q \circ k}$ & 59.11 & 40.61 \\ % #1
Prob diff & $\Pqa{a^* | q \circ k} - \Pqa{a^* | q}$ & \textbf{60.69} & 40.91 \\ % #0
Score diff & $\Sqa{a^* | q \circ k} - \Sqa{a^* | q}$ & 58.26 & 39.86 \\ % #2
% \quad Unif. ref. & $\frac{1}{2} \Big[ \tanh \big( \Pqa{a^* | q \circ k} - \frac{1}{|A|} \big) - \tanh \big( \Pqa{a^* | q} - \frac{1}{|A|} \big) \Big]$ & 58.90 & 40.25 \\ % #6
Hard activation & $\frac{1}{2} \Big[ \sgn \big( \Sqa{a^* | q \circ k} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q \circ k} \big)$ \\ & $\qquad - \sgn \big( \Sqa{a^* | q} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q} \big) \Big]$ & 58.32 & 41.16 \\ % #5
\bottomrule
\end{tabular}
}%
\vspace{-4pt}
\caption{
    Ablations on the choice of reward function.
    % \hanna{the prob. diff also gives really good results and it is pretty easier and more intuititve, no? do you want to argue why you need the hyperbolic reward shaping?}
}
\label{tab:ablation_rewards}
\end{minipage}
\vspace{-8pt}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/human.tex <==
\begin{figure*}
\begin{minipage}{.22\linewidth}
\centering
\includegraphics[width=\linewidth]{images/human_bar.png}
\end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
\centering
\includegraphics[width=\linewidth]{images/human_pie.png}
\end{minipage}
\hfill
\begin{minipage}{.28\linewidth}
\centering
\includegraphics[width=\linewidth]{images/human_cats.png}
\end{minipage}
\caption{
    Human analysis of \methodname{}-generated knowledge.
    \textbf{Left:} Percentage of good knowledge in each quality aspect.
    \textbf{Mid:} Agreement between human and machine on helpfulness of \textit{selected knowledge}.
    \textbf{Right:} Percentage of \methodname{}-generated knowledge categorized by domain, expressed relation, and syntax. The percentages do not add up to 100\% because some knowledge have none of these characteristics, while some others may have multiple.
}
\label{fig:human}
\vspace{-8pt}
\end{figure*}

==> [EMNLP 2022] cc-GKM/floats/hypers.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{c c l}
\toprule
\textbf{Symbol} & \textbf{Value} & \textbf{Description} \\
\midrule
\multicolumn{3}{c}{\textsc{Getting Silver Knowledge from Few-Shot GPT-3}} \\
\midrule
$M$ & 20 & Number of knowledge statements to sample from GPT-3, per question. \\
$p$ & 0.5 & Parameter for nucleus sampling from GPT-3. \\
$L_{\text{output}}$ & 64 & Max length of output from GPT-3. \\
\midrule
\multicolumn{3}{c}{\textsc{Stage I: Imitation Learning}} \\
\midrule
$L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
$L_{\text{output}}$ & 64 & Max length of output from \methodname{} (i.e. generated knowledge). \\
$B$ & 64 & Batch size for training. \\
$S$ & 50,000 & Total number of training steps. \\
$\eta$ & $1 \times 10^{-5}$ & Learning rate of Adam optimizer. \\
\midrule
\multicolumn{3}{c}{\textsc{Stage II: Reinforcement Learning}} \\
\midrule
$\alpha$ & 1.0 & Weight of value model loss in PPO. \\
$\beta$ & 0.2 & Weight of entropy bonus term in reward. \\
$\gamma$ & 1.0 & Discount factor for rewards. \\
$\lambda$ & 0.95 & Parameter for advantage estimation. \\
$\eps$ & 0.2 & Clipping range for the \textit{clipped surrogate objective}. \\
$L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
$L_{\text{output}}$ & 32 & Max length of output from \methodname{} (i.e. generated knowledge). \\
$\tau$ & 0.7 & Temperature for knowledge sampling in PPO training. \\
$E$ & 1M & Total number of training episodes. \\
$B$ & 64 & Batch size for training. \\
$S$ & 15,625 & Total number of training steps. \\
$s$ & 4 & Interval (in steps) for updating the lagging models (policy and value). \\
$\eta$ & $2 \times 10^{-5}$ & Learning rate of Adam optimizer (with a linear learning rate decay schedule). \\
\midrule
\multicolumn{3}{c}{\textsc{Inference}} \\
\midrule
$M$ & 10 & Number of knowledge statements to sample from \methodname{}, per question. \\
$p$ & 0.5 & Parameter for nucleus sampling from \methodname{}. \\
$L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
$L_{\text{output}}$ & 32 & Max length of output from \methodname{}. \\
\bottomrule
\end{tabular}
\caption{Hyperparameter settings.}
\label{tab:hypers}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/ppo.tex <==
\begin{figure}[t]
\begin{algorithm}[H]
\footnotesize
\caption{
    Training \methodname{}
}
% \hanna{if you ran out of space; you can easily remove procedure getweakannotation adn imitation learning. Just in the main text write "GetWeakannotation (...) from eq1; you can do the same thing for imitationlearning.}
\textbf{Input} initial policy model $\theta_0$, initial value model $\phi_0$, pre-trained QA model $\psi_{\text{QA}}$ \\
 \hspace*{2mm} $\Ds_{\text{imit}} \gets$ Get silver knowledge on $\Ds_{\text{seen}}$ from GPT-3. \\
  \hspace*{2mm} $\theta_{\text{imit}} \gets$ Optimize $\theta_0$ with Eqn~\ref{eqn:imit-loss} from $\Ds_{\text{imit}}$. \algorithmiccomment{Section \ref{sec:method_imit}} \\
   \hspace*{2mm} $\theta_{\methodname{}} \gets$ \Call{ReinforcedLearning}{$\Ds_{\text{seen}}$, $\theta_{\text{imit}}$, $\phi_0$, $\psi_{\text{QA}}$} \\
\hspace*{2mm} \phantom{...} \algorithmiccomment{Section \ref{sec:method_rl}} 
\begin{algorithmic}
%\Procedure{\textcolor{brown}{Train\methodname{}}}{$\Ds_{\text{ID}}$, \textit{base\_model}, \textit{QA\_model}}
    % \State $\theta_0 \gets$ the parameterization of pre-trained \textit{base\_model}
    % \State $\phi_0 \gets$ the parameterization of pre-trained \textit{base\_model}
%    \State \dif{Initialize $\theta_0$ and $\phi_0$ with the pre-trained \textit{base\_model}}
    % \yejin{why definition repeats for two different variables?} \gary{Because the policy and value models are initialized from the same pre-trained LM.}
    % \State $\psi_{\text{QA}} \gets$ the parameterization of pre-trained \textit{QA\_model}
%    \State Initialize $\psi_{\text{QA}}$ with the pre-trained \textit{QA\_model}
%    \State $\Ds_{\text{imit}} \gets$ Get silver knowledge on $\Ds_{\text{ID}}$ with GPT-3.
%    \State $\theta_{\text{imit}} \gets$ \Call{\textcolor{teal}{ImitationLearning}}{$\Ds_{\text{imit}}$, $\theta_0$}
%    \State $\theta_{\methodname{}} \gets$ \Call{\textcolor{violet}{ReinforcedLearning}}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\phi_0$, $\psi_{\text{QA}}$}
%    \State \Return $\theta_{\methodname{}}$
%\EndProcedure
% \Procedure{GetWeakAnnotationFromGPT3}{$\Ds_{\text{ID}}$}
%     \State Construct $\Ds_{\text{imit}}$ with Eqn~\ref{eqn:Dimit-construction} and return it.
%     % \State $\Ds_{\text{imit}} \gets \{\}$
%     % \ForAll {$(q, A, a^*) \in \Ds_{\text{ID}}$}
%     %     \For {$m = 1 \hdots M$}
%     %         \State $k \gets$ \Call{NucleusSampling}{$q$, prompt(task($q$)), GPT-3, $p$}
%     %         \State $\Ds_{\text{imit}} \gets \Ds_{\text{imit}} \cup \{ (q, k) \}$
%     %     \EndFor
%     % \EndFor
%     % \State \Return $\Ds_{\text{imit}}$
% \EndProcedure
%\Procedure{\textcolor{teal}{ImitationLearning}}{$\Ds_{\text{imit}}$, $\theta_0$}
 %   \State Optimize $\theta_0$ with Eqn~\ref{eqn:imit-loss} from $\Ds_{\text{imit}}$.
    % \For {$i = 1 \hdots S$}
    %     \State \textit{batch} $\gets$ sample a batch of size $B$ from $\Ds_{\text{imit}}$
    %     \State $\theta \gets \theta - \eta \cdot \nabla_\theta \frac{1}{B} \sum_{(q, k) \in \textit{batch}}{-\log{p_K(k | q; \theta)} / |k|}$
    % \EndFor
 %   \State \Return $\theta$
%\EndProcedure
\Procedure{ReinforcedLearning}{$\Ds_{\text{seen}}$, $\theta$, $\phi$, $\psi_{\text{QA}}$}
    % \Procedure{ComputeRewardNormalizationFactors}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\psi_{\text{QA}}$}
    %     \State $\mathcal{R}_{\text{init}} \gets \{\}$
    %     \ForAll {$x = (q, A, a^*) \in \Ds_{\text{ID}}$}
    %         \State $k \gets$ \Call{TemperatureSampling}{$q$, $\theta_{\text{imit}}$, $\tau$}
    %         \State $r \gets r(x, k; \psi_{\text{QA}})$
    %         \State $\mathcal{R}_{\text{init}} \gets \mathcal{R}_{\text{init}} \cup \{ r \}$
    %     \EndFor
    %     \State $\mu_0 \gets \mu(\mathcal{R}_{\text{init}})$, $\sigma_0 \gets \sigma(\mathcal{R}_{\text{init}})$
    %     \State \Return $(\mu_0, \sigma_0)$
    % \EndProcedure
    % \State $(\mu_0, \sigma_0) \gets$ \Call{ComputeRewardNormalizationFactors}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\psi_{\text{QA}}$}
    %\State $(\mu_0, \sigma_0) \gets$ Compute reward norm factors with Eqn~\ref{eqn:reward-norm-compute}.
    \State $\theta_{\text{old}} \gets \theta$, $\phi_{\text{old}} \gets \phi$
    % \For {$i = 1 \hdots S$}
        % \State \textit{batch} $\gets$ sample a batch of size $B$ from $\Ds_{\text{ID}}$
        % \State $\mathcal{L}_{\text{Policy}} \gets 0$, $\mathcal{L}_{\text{Value}} \gets 0$
        % \ForAll {$(q, A, a^*) \in$ \textit{batch}}
        %     \State $k \gets$ \Call{TemperatureSampling}{$q$, $\theta$, $\tau$}
        %     \State $r \gets r(x, k; \psi_{\text{QA}})$
        %     \State $r \gets (r - \mu_0) / \sigma_0$
        %     \State $R \gets r - \beta \log{\big( p_K(k | q; \theta) / p_K(k | q; \theta_{\text{imit}}) \big)}$
        %     \State $T \gets |k|$
        %     \State $r_T \gets R$, $r_{[1 \hdots T-1]} \gets 0$
        %     \For {$t = T \hdots 1$}
        %         \State $\delta_t \gets r_t + \gamma V(s_{t+1}; \phi) - V(s_t; \phi)$
        %         \State $\hat{A}_t \gets \delta_t + (\gamma \lambda) \delta_{t+1} + \hdots + (\gamma \lambda)^{T-t+1} \delta_{T-1}$
        %         \State $V_t^{\text{targ}} \gets r_t + \gamma r_{t+1} + \hdots + \gamma^{T-t+1} r_{T-1} + \gamma^{T-t} V(s_T; \phi_{\text{old}})$
        %         \State $\nu_t \gets p_K(k_t | q; \theta) / p_K(k_t | q; \theta_{\text{old}})$
        %         \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} - \min \big( \nu_t \hat{A}_t, \text{clip}(\nu_t, 1 - \eps, 1 + \eps) \hat{A}_t \big)$
        %         \State $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} + (V(s_t; \phi) - V_t^{\text{targ}})^2$
        %     \EndFor
        %     \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} / T$, $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} / T$
        % \EndFor
        % \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} / B$, $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} / B$
        % \State $\mathcal{L}_{\text{PPO}} \gets \mathcal{L}_{\text{Policy}} + \alpha \cdot \mathcal{L}_{\text{Value}}$
    \For{iterations = 1, 2, \ldots}
        \State Sample a minibatch from $\Ds_{\text{seen}}$.
        \For{step = 1, 2, \ldots, $s$}
            \State Compute $\mathcal{L}_{\text{PPO}}$ on the minibatch with Eqn~\ref{eqn:ppo-loss}.
        % \State $\theta \gets \theta - \eta \cdot \nabla_\theta \mathcal{L}_{\text{PPO}}$, $\phi \gets \phi - \eta \cdot \nabla_\phi \mathcal{L}_{\text{PPO}}$
            \State Optimize $\theta$ and $\phi$ with $\mathcal{L}_{\text{PPO}}$ for one step.
        % \If {$i \equiv 0 (\text{mod } s)$} \Comment{Update the lagging policy every $s$ steps.}
        %\If {$s$ minibatches has elapsed \dif{since the last update on the lagging models}}
        % \yejin{not sure what 'last lagging model update' means, and in any case, this phrase might not be grammatically correct}
        %\EndIf
        \EndFor
        \State $\theta_{\text{old}} \gets \theta$, $\phi_{\text{old}} \gets \phi$
    \EndFor
    \State \Return $\theta$
\EndProcedure
\end{algorithmic}
\textbf{Output} $\theta_{\methodname{}}$
\label{alg:ppo}
\end{algorithm}
% \vspace{-24pt}
% \caption{\ximing{working on a new version of algorithm 1}}
\end{figure}

% \begin{figure}[t]
% \begin{algorithm}[H]
% \footnotesize
% \caption{
%     Training \methodname{}
% }
% % \hanna{if you ran out of space; you can easily remove procedure getweakannotation adn imitation learning. Just in the main text write "GetWeakannotation (...) from eq1; you can do the same thing for imitationlearning.}
% \begin{algorithmic}
% \Procedure{Train\methodname{}}{$\Ds_{\text{ID}}$, \textit{base\_model}, \textit{QA\_model}}
%     % \State $\theta_0 \gets$ the parameterization of pre-trained \textit{base\_model}
%     % \State $\phi_0 \gets$ the parameterization of pre-trained \textit{base\_model}
%     \State \dif{Initialize $\theta_0$ and $\phi_0$ with the pre-trained \textit{base\_model}}
%     % \yejin{why definition repeats for two different variables?} \gary{Because the policy and value models are initialized from the same pre-trained LM.}
%     % \State $\psi_{\text{QA}} \gets$ the parameterization of pre-trained \textit{QA\_model}
%     \State Initialize $\psi_{\text{QA}}$ with the pre-trained \textit{QA\_model}
%     \State $\Ds_{\text{imit}} \gets$ Get silver knowledge on $\Ds_{\text{ID}}$ with GPT-3.
%     \State $\theta_{\text{imit}} \gets$ \Call{ImitationLearning}{$\Ds_{\text{imit}}$, $\theta_0$}
%     \State $\theta_{\methodname{}} \gets$ \Call{ReinforcedLearning}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\phi_0$, $\psi_{\text{QA}}$}
%     \State \Return $\theta_{\methodname{}}$
% \EndProcedure
% % \Procedure{GetWeakAnnotationFromGPT3}{$\Ds_{\text{ID}}$}
% %     \State Construct $\Ds_{\text{imit}}$ with Eqn~\ref{eqn:Dimit-construction} and return it.
% %     % \State $\Ds_{\text{imit}} \gets \{\}$
% %     % \ForAll {$(q, A, a^*) \in \Ds_{\text{ID}}$}
% %     %     \For {$m = 1 \hdots M$}
% %     %         \State $k \gets$ \Call{NucleusSampling}{$q$, prompt(task($q$)), GPT-3, $p$}
% %     %         \State $\Ds_{\text{imit}} \gets \Ds_{\text{imit}} \cup \{ (q, k) \}$
% %     %     \EndFor
% %     % \EndFor
% %     % \State \Return $\Ds_{\text{imit}}$
% % \EndProcedure
% \Procedure{ImitationLearning}{$\Ds_{\text{imit}}$, $\theta_0$}
%     \State $\theta \gets \theta_0$
%     \State Optimize $\theta$ with Eqn~\ref{eqn:imit-loss} for $S$ minibatches from $\Ds_{\text{imit}}$.
%     % \For {$i = 1 \hdots S$}
%     %     \State \textit{batch} $\gets$ sample a batch of size $B$ from $\Ds_{\text{imit}}$
%     %     \State $\theta \gets \theta - \eta \cdot \nabla_\theta \frac{1}{B} \sum_{(q, k) \in \textit{batch}}{-\log{p_K(k | q; \theta)} / |k|}$
%     % \EndFor
%     \State \Return $\theta$
% \EndProcedure
% \Procedure{ReinforcedLearning}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\phi_0$, $\psi_{\text{QA}}$}
%     % \Procedure{ComputeRewardNormalizationFactors}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\psi_{\text{QA}}$}
%     %     \State $\mathcal{R}_{\text{init}} \gets \{\}$
%     %     \ForAll {$x = (q, A, a^*) \in \Ds_{\text{ID}}$}
%     %         \State $k \gets$ \Call{TemperatureSampling}{$q$, $\theta_{\text{imit}}$, $\tau$}
%     %         \State $r \gets r(x, k; \psi_{\text{QA}})$
%     %         \State $\mathcal{R}_{\text{init}} \gets \mathcal{R}_{\text{init}} \cup \{ r \}$
%     %     \EndFor
%     %     \State $\mu_0 \gets \mu(\mathcal{R}_{\text{init}})$, $\sigma_0 \gets \sigma(\mathcal{R}_{\text{init}})$
%     %     \State \Return $(\mu_0, \sigma_0)$
%     % \EndProcedure
%     % \State $(\mu_0, \sigma_0) \gets$ \Call{ComputeRewardNormalizationFactors}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\psi_{\text{QA}}$}
%     \State $(\mu_0, \sigma_0) \gets$ Compute reward norm factors with Eqn~\ref{eqn:reward-norm-compute}.
%     \State $\theta \gets \theta_{\text{imit}}$, $\phi \gets \phi_0$
%     \State $\theta_{\text{old}} \gets \theta$, $\phi_{\text{old}} \gets \phi$
%     % \For {$i = 1 \hdots S$}
%         % \State \textit{batch} $\gets$ sample a batch of size $B$ from $\Ds_{\text{ID}}$
%         % \State $\mathcal{L}_{\text{Policy}} \gets 0$, $\mathcal{L}_{\text{Value}} \gets 0$
%         % \ForAll {$(q, A, a^*) \in$ \textit{batch}}
%         %     \State $k \gets$ \Call{TemperatureSampling}{$q$, $\theta$, $\tau$}
%         %     \State $r \gets r(x, k; \psi_{\text{QA}})$
%         %     \State $r \gets (r - \mu_0) / \sigma_0$
%         %     \State $R \gets r - \beta \log{\big( p_K(k | q; \theta) / p_K(k | q; \theta_{\text{imit}}) \big)}$
%         %     \State $T \gets |k|$
%         %     \State $r_T \gets R$, $r_{[1 \hdots T-1]} \gets 0$
%         %     \For {$t = T \hdots 1$}
%         %         \State $\delta_t \gets r_t + \gamma V(s_{t+1}; \phi) - V(s_t; \phi)$
%         %         \State $\hat{A}_t \gets \delta_t + (\gamma \lambda) \delta_{t+1} + \hdots + (\gamma \lambda)^{T-t+1} \delta_{T-1}$
%         %         \State $V_t^{\text{targ}} \gets r_t + \gamma r_{t+1} + \hdots + \gamma^{T-t+1} r_{T-1} + \gamma^{T-t} V(s_T; \phi_{\text{old}})$
%         %         \State $\nu_t \gets p_K(k_t | q; \theta) / p_K(k_t | q; \theta_{\text{old}})$
%         %         \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} - \min \big( \nu_t \hat{A}_t, \text{clip}(\nu_t, 1 - \eps, 1 + \eps) \hat{A}_t \big)$
%         %         \State $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} + (V(s_t; \phi) - V_t^{\text{targ}})^2$
%         %     \EndFor
%         %     \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} / T$, $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} / T$
%         % \EndFor
%         % \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} / B$, $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} / B$
%         % \State $\mathcal{L}_{\text{PPO}} \gets \mathcal{L}_{\text{Policy}} + \alpha \cdot \mathcal{L}_{\text{Value}}$
%     \For {$S$ minibatches from $\Ds_{\text{ID}}$}
%         \State Compute $\mathcal{L}_{\text{PPO}}$ on the minibatch with Eqn~\ref{eqn:ppo-loss}.
%         % \State $\theta \gets \theta - \eta \cdot \nabla_\theta \mathcal{L}_{\text{PPO}}$, $\phi \gets \phi - \eta \cdot \nabla_\phi \mathcal{L}_{\text{PPO}}$
%         \State Optimize $\theta$ and $\phi$ with $\mathcal{L}_{\text{PPO}}$ for one step.
%         % \If {$i \equiv 0 (\text{mod } s)$} \Comment{Update the lagging policy every $s$ steps.}
%         \If {$s$ minibatches has elapsed \dif{since the last update on the lagging models}}
%         % \yejin{not sure what 'last lagging model update' means, and in any case, this phrase might not be grammatically correct}
%             \State $\theta_{\text{old}} \gets \theta$, $\phi_{\text{old}} \gets \phi$
%         \EndIf
%     \EndFor
%     \State \Return $\theta$
% \EndProcedure
% \end{algorithmic}
% \label{alg:ppo}
% \end{algorithm}
% \vspace{-24pt}
% \end{figure}

==> [EMNLP 2022] cc-GKM/floats/prompts/ai2sci.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
\midrule
AI2Sci & Input: Which is a nonrenewable natural resource that is used to make electrical energy? \textbackslash{}n (A) coal (B) wind (C) water (D) thermal \\
& Knowledge: \textbf{Fossil fuel is nonrenewable natural resource.} \\
\\
& Input: Which adaptation will warn predators not to eat an animal? \textbackslash{}n (A) bright colors (B) bulging eyes (C) geometric shapes (D) poisonous secretions \\
& Knowledge: \textbf{Bright colors in animals are usually a sign of being poisonous.} \\
\\
& Input: An Italian scientist named Alessandro Volta invented the Voltaic pile in 1800. It was able to produce a steady electrical current. Based on this description, what is the modern equivalent of the Voltaic pile? \textbackslash{}n (A) a wire (B) a battery (C) a resistor (D) a light bulb \\
& Knowledge: \textbf{Batteries can produce steady electrical current.} \\
\\
& Input: What is the best measure to use in determining the effect of solar energy on Earth's atmosphere? \textbackslash{}n (A) the temperature of the air (B) the temperature of the ocean (C) the density of clouds in the sky (D) the amount of rainfall on a rainy day \\
& Knowledge: \textbf{Solar radiation converts to heat in Earth's atmosphere.} \\
\\
& Input: Which nongaseous compound can be made from two elements that are gases at room temperature? \textbackslash{}n (A) water (B) table salt (C) iron oxide (D) carbon dioxide \\
& Knowledge: \textbf{Water molecules are made of Hydrogen and Oxygen.} \\
\\
& Input: \{question\}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for AI2Science.
}
\label{tab:prompt_ai2sci}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/prompts/arc.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
\midrule
ARC & Input: George wants to warm his hands quickly by rubbing them. Which skin surface will produce the most heat? \textbackslash{}n (A) dry palms (B) wet palms (C) palms covered with oil (D) palms covered with lotion \\
& Knowledge: \textbf{Rubbing hands produces heat because of friction.} \\
\\
& Input: Which of the following is an example of a physical change? \textbackslash{}n (A) lighting a match (B) breaking a glass (C) burning of gasoline (D) rusting of iron \\
& Knowledge: \textbf{Physical changes must not involve chemical changes such as combustion and rusting.} \\
\\
& Input: On Earth, water can be a solid, a liquid, or a gas. Which energy source has the greatest influence on the state of matter of water? \textbackslash{}n (A) the sun (B) the wind (C) ocean currents (D) the metal core \\
& Knowledge: \textbf{Earth's water circulation is mostly driven by heat radiated from the sun.} \\
\\
& Input: What do cells break down to produce energy? \textbackslash{}n (A) food (B) water (C) chlorophyll (D) carbon dioxide \\
& Knowledge: \textbf{Food contain calories.} \\
\\
& Input: What characteristic of DNA results in cell differentiation in developing embryos? \textbackslash{}n (A) which genes are present (B) how many copies of each gene are present (C) which genes are active (D) what protein is produced by a gene \\
& Knowledge: \textbf{Cell differentiation is caused by selective expression of genes.} \\
\\
& Input: \{question\}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for ARC.
}
\label{tab:prompt_arc}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/prompts/csqa.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
\midrule
CSQA & Input: Google Maps and other highway and street GPS services have replaced what? \textbackslash{}n (A) united states (B) mexico (C) countryside (D) atlas (E) oceans \\
& Knowledge: \textbf{Electronic maps are the modern version of paper atlas.} \\
\\
& Input: The fox walked from the city into the forest, what was it looking for? \textbackslash{}n (A) pretty flowers. (B) hen house (C) natural habitat (D) storybook (E) dense forest \\
& Knowledge: \textbf{Natural habitats are usually away from cities.} \\
\\
& Input: You can share files with someone if you have a connection to a what? \textbackslash{}n (A) freeway (B) radio (C) wires (D) computer network (E) electrical circuit \\
& Knowledge: \textbf{Files can be shared over the Internet.} \\
\\
& Input: Too many people want exotic snakes.  The demand is driving what to carry them? \textbackslash{}n (A) ditch (B) shop (C) north america (D) pet shops (E) outdoors \\
& Knowledge: \textbf{Some people raise snakes as pets.} \\
\\
& Input: The body guard was good at his duties, he made the person who hired him what? \textbackslash{}n (A) better job (B) irritated (C) feel safe (D) save money (E) headache \\
& Knowledge: \textbf{The job of body guards is to ensure the safety and security of the employer.} \\
\\
& Input: \{question\}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for CommonsenseQA.
}
\label{tab:prompt_csqa}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/prompts/obqa.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
\midrule
OBQA & Input: The sun is responsible for \textbackslash{}n (A) puppies learning new tricks (B) children growing up and getting old (C) flowers wilting in a vase (D) plants sprouting, blooming and wilting \\
& Knowledge: \textbf{Natural light provides energy for photosynthesis.} \\
\\
& Input: Poison causes harm to which of the following? \textbackslash{}n (A) a Tree (B) a robot (C) a house (D) a car \\
& Knowledge: \textbf{Living organisms are susceptible to poisonous matter.} \\
\\
& Input: As a car approaches you in the night \textbackslash{}n (A) the headlights become more intense (B) the headlights recede into the dark (C) the headlights remain at a constant (D) the headlights turn off \\
& Knowledge: \textbf{The intensity of light increases when observed from a shorter distance.} \\
\\
& Input: When the weather changes as it does from Christmas to Easter, \textbackslash{}n (A) the air may chill (B) the ground may freeze (C) the plants may die (D) the ground may warm \\
& Knowledge: \textbf{Christmas is in winter and Easter is in spring.} \\
\\
& Input: Using mirrors to focus collected light from heavenly bodies allows \textbackslash{}n (A) detailed observation (B) foregone conclusions (C) radiation experiments (D) celestial music \\
& Knowledge: \textbf{Telescopes use mirrors to focus light from the stars.} \\
\\
& Input: \{question\}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for OpenBookQA.
}
\label{tab:prompt_obqa}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/prompts/piqa.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
\midrule
PIQA & Input: how do you flood a room? \textbackslash{}n (A) fill it with objects. (B) fill it with water. \\
& Knowledge: \textbf{Too much water can cause flooding.} \\
\\
& Input: How can I get oil stains out of my driveway? \textbackslash{}n (A) Douse each stain with a couple cans of beer. (B) Douse each stain with a couple cans of soda. \\
& Knowledge: \textbf{Sodium carbonate solution can wash away oil stains.} \\
\\
& Input: Soothe a painful sunburn. \textbackslash{}n (A) Wait until brewed tea bag is cool, then apply on burn. (B) Wait until brewed tea bag is hot, then apply on burn. \\
& Knowledge: \textbf{Sunburn can be alleviated by applying cold material.} \\
\\
& Input: What can I use for fuel in an alcohol stove? \textbackslash{}n (A) Use acetone. (B) Use vinegar. \\
& Knowledge: \textbf{Acetone is flammable, while vinegar is not.} \\
\\
& Input: How can I cut the handles of metal cutlery? \textbackslash{}n (A) Use a hand saw to cut the handles. (B) Use a hand drill to cut the handles. \\
& Knowledge: \textbf{A hand saw is used for making cuts; a hand drill is used for making holes.} \\
\\
& Input: \{question\}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for PhysicalIQA.
}
\label{tab:prompt_piqa}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/prompts/qasc.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
\midrule
QASC & Input: What type of water formation is formed by clouds? \textbackslash{}n (A) pearls (B) streams (C) shells (D) diamonds (E) rain (F) beads (G) cooled (H) liquid \\
& Knowledge: \textbf{Clouds are made of water vapor.} \\
\\
& Input: What can prevent food spoilage? \textbackslash{}n (A) prolactin release (B) one celled organisms (C) hydrating food (D) cleaning food (E) airing out food (F) Electric generators (G) a hydraulic system (H) dehydrating food \\
& Knowledge: \textbf{Dehydrating food is used for preserving food.} \\
\\
& Input: The process by which genes are passed is \textbackslash{}n (A) Most plants (B) flow of electrons (C) mitosis (D) Summer (E) respiration (F) mutation (G) mechanical (H) reproduction \\
& Knowledge: \textbf{Genes are passed from parent to offspring.} \\
\\
& Input: The stomach does what in the body? \textbackslash{}n (A) decreases its bodily water (B) kills all germs (C) breaks food into nutrients (D) stores bile (E) heat is produced (F) extracts water from food (G) get chemical reactions started (H) cause people to become sick. \\
& Knowledge: \textbf{The stomach is part of the digestive system.} \\
\\
& Input: What can cause rocks to break down? \textbackslash{}n (A) Wind Barriers (B) Protective Barriers (C) Stone Sealers (D) wind (E) mines (F) Water (G) erosion (H) Gravity \\
& Knowledge: \textbf{Mechanical weathering is when rocks are broken down by mechanical means.} \\
\\
& Input: \{question\}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for QASC.
}
\label{tab:prompt_qasc}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/prompts/siqa.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
\midrule
SIQA & Input: What will Quinn want to do next? \textbackslash{}n (A) Eat messy snacks (B) help out a friend (C) Pick up the dirty clothes \textbackslash{}n Quinn wanted to help me clean my room up because it was so messy. \\
& Knowledge: \textbf{A messy room likely contains dirty clothes.} \\
\\
& Input: What will Aubrey want to do next? \textbackslash{}n (A) help Aubrey go back home (B) keep on partying without the mom (C) going on with the mom \textbackslash{}n Sasha's mom passed out in the middle of the party. Aubrey took Sasha's mom to the hospital. \\
& Knowledge: \textbf{One should attend to their sick family member.} \\
\\
& Input: How would Jan feel afterwards? \textbackslash{}n (A) scared of losing the cat (B) normal (C) relieved for fixing the problem \textbackslash{}n Their cat kept trying to escape out of the window, so Jan placed an obstacle in the way. \\
& Knowledge: \textbf{One usually has positive emotions after solving a problem.} \\
\\
& Input: How would Sydney feel afterwards? \textbackslash{}n (A) affected (B) like they released their tension (C) worse \textbackslash{}n Sydney had so much pent up emotion, they burst into tears at work. \\
& Knowledge: \textbf{Crying can be a catharsis.} \\
\\
& Input: What does Sydney need to do before this? \textbackslash{}n (A) be bad at her job (B) do a good job (C) be lazy \textbackslash{}n Sydney got a raise and a new promotion. \\
& Knowledge: \textbf{Pay raise and promotion are usually results of good job performance.} \\
\\
& Input: \{question\}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for SocialIQA.
}
\label{tab:prompt_siqa}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/prompts/wg.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
\midrule
WG & Input: The GPS and map helped me navigate home.  I got lost when the \_ got turned off. \textbackslash{}n (A) GPS (B) map \\
& Knowledge: \textbf{A GPS device is electronic, while a map is paper-based.} \\
\\
& Input: I picked up a bag of peanuts and raisins for a snack. I wanted a sweeter snack out so I ate the \_ for now. \textbackslash{}n (A) raisins (B) peanuts \\
& Knowledge: \textbf{Peanuts contain a lot of fat. Raisins contain a lot of sugar.} \\
\\
& Input: The geese prefer to nest in the fields rather than the forests because in the \_ predators are more hidden. \textbackslash{}n (A) fields (B) forests \\
& Knowledge: \textbf{There are more trees in the forests than in the fields.} \\
\\
& Input: Once in Poland, Dennis enjoyed the trip more than Jason because \_ had a shallow understanding of the Polish language. \textbackslash{}n (A) Dennis (B) Jason \\
& Knowledge: \textbf{Those who know the native language would enjoy the trip better.} \\
\\
& Input: Adam put handwash only clothes in the washer but Aaron washed them by hand as \_ was lazy. \textbackslash{}n (A) Adam (B) Aaron \\
& Knowledge: \textbf{Washing clothes with washer takes less effort than by hand.} \\
\\
& Input: \{question\}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for Winogrande.
}
\label{tab:prompt_wg}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/qual.tex <==
\begin{table*}
\setlength{\tabcolsep}{3pt}
\footnotesize
\centering
\begin{tabular}{cp{280pt} p{32pt}p{40pt}p{40pt}}
\toprule
\textbf{Task} & Question / \textbf{Knowledge} & \textbf{Domain} & \textbf{Relation} & \textbf{Syntax} \\
\midrule
\multirow{2}{*}{CSQA} & What would vinyl be an odd thing to replace? (A) pants (B) record albums (C) record store (D) cheese \Right{(E) wallpaper} \\
& \qquad \textbf{Vinyl is a type of plastic.} & scientific & member of & -- \\
\midrule
\multirow{2}{*}{QASC} & Some pelycosaurs gave rise to reptile ancestral to (A) lamphreys (B) angiosperm \Right{(C) mammals} (D) paramecium (E) animals (F) protozoa (G) arachnids (H) backbones & \quad \newline \quad \newline scientific \\
& \qquad \textbf{Reptiles are the ancestors of all mammals.} & temporal & attribute & -- \\
% \midrule
% \multirow{2}{*}{QASC} & What are aquatic animals? \newline (A) Pelycosaur (B) candy (C) water (D) angiosperm \newline (E) weater \Right{(F) jellyfish} (G) arachnids (H) cookies \\
% & \qquad \textbf{Aquatic animals are animals that swim.} & scientific & attribute & -- \\
% \midrule
% \multirow{2}{*}{PIQA} & To discourage house flies from living in your home, \Right{(A) keep basil plants in the kitchen or windows.} (B) keep lavender plants in the kitchen or window. \\ % This example is WRONG
% & \qquad \textbf{Lavender is a deterrent to house flies.} & scientific & attribute & -- \\
\midrule
\multirow{2}{*}{SIQA} & Sydney rubbed Addison's head because she had a horrible headache. What will happen to Sydney? (A) drift to sleep \Right{(B) receive thanks} (C) be reprimanded \\
& \qquad \textbf{A good deed will be rewarded.} & social & -- & -- \\
% \midrule
% \multirow{2}{*}{WG} & Sarah rolls her eyes as Monica extolls the virtues of vinegar as a cleaning solution for everything since \_ is bored. \newline \Right{(A) Sarah} (B) Monica \\
% & \qquad \textbf{Monica is a good teacher.} & social & attribute & -- \\
\midrule
\multirow{2}{*}{WG} & Adam always spent all of the free time watching Tv unlike Hunter who volunteered, due to \_ being lazy. \Right{(A) Adam} (B) Hunter \\
& \qquad \textbf{Hunter is more active than Adam.} & social & attribute & comparison \\
% \midrule
% \multirow{2}{*}{RS} & What can you share and still have all for yourself? \newline (A) cut \Right{(B) knowledge} (C) humans (D) freedom (E) valence \\
% & \qquad \textbf{You can share knowledge and still have all for yourself.} & -- & -- & -- \\
\midrule
\multirow{2}{*}{RS} & Causes bad breath and frightens blood-suckers (A) tuna (B) iron (C) trash \Right{(D) garlic} (E) pubs \\
& \qquad \textbf{Garlic is a strong-smelling food.} & -- & attribute & -- \\
\midrule
\multirow{2}{*}{QuaRTz} & If the mass of an object gets bigger what will happen to the amount of matter contained within it? \Right{(A) gets bigger} (B) gets smaller & \quad \newline scientific \\
& \quad \textbf{The mass of an object is proportional to the amount of matter it contains.} & physical & -- & -- \\
\bottomrule
\end{tabular}
\caption{
    Examples of good knowledge generated by \methodname{}.
    Each of these knowledge rectifies UnifiedQA-large's prediction, and is labeled by the annotator as relevant, factual, and helpful.
}
\label{tab:qual}
\vspace{-8pt}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/qual_culture.tex <==
\begin{table*}[h!]
\setlength{\tabcolsep}{3pt}
\footnotesize
\centering
\begin{tabular}{cp{200pt} p{144pt}}
\toprule
\textbf{Task} & Question / \textbf{Knowledge} & \textbf{Problem with the knowledge} \\
\midrule
SIQA & Remy made hay getting home from school on Friday the 13th. Why did Remy do this? \newline (A) go to school before this (B) had heard that on Friday the 13th, God would bless you if you just went home and hid \Right{(C) had heard that on Friday the 13th, that people pranked other people really bad} \newline \textbf{People are more likely to be pranked on Friday the 13th.} & \textbf{Culture-specific} \newline This knowledge largely applies within western, especially Christian, culture. \\
\midrule
WG & Lindsey like to read graphic novels but Natalie liked classic literature to read. \_ bought the new Frank Miller comic at the book store. \newline \Right{(A) Lindsey} (B) Natalie \newline \textbf{Graphic novels are popular among teens.} & \textbf{Culture-specific} \newline This knowledge could be correct or not depending on the culture or geographical location. \\
\midrule
CSQA & Where would a person live that isn't in the metro area but still has good schools? \newline (A) woods (B) bed \Right{(C) suburbs} (D) rural (E) neighborhood \newline \textbf{A person who lives in the suburbs is likely to have good schools.} & \textbf{Culture-specific} \newline This knowledge could be correct or not depending on the culture or geographical location, and it is not even always true within the U.S. \\
\midrule
NS & most people in the u.s. works <mask> consecutive hours in a business day. \newline (A) no (B) one (C) two (D) three (E) four (F) five (G) six (H) seven \Right{(I) eight} (J) nine (K) ten \newline \textbf{Most people work eight hours in a day.} & \textbf{Culture-specific} \newline This knowledge is an over-generalization. In some other cultures, most people work more then eight hours, or less. \\
\midrule
CSQA & What will god never do according to religion? \newline (A) anything \Right{(B) judge people} (C) work miracles (D) judge men (E) everywhere \newline \textbf{God is a judge of people.} & \textbf{Culture-specific} \newline This is a topic specific to the religion. \\
\bottomrule
\end{tabular}
\caption{
    Examples of knowledge generated by \methodname{} that are culture-specific.
}
\label{tab:qual_culture}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/qual_ethics.tex <==
\begin{table*}[h!]
\setlength{\tabcolsep}{3pt}
\footnotesize
\centering
\begin{tabular}{cp{200pt} p{144pt}}
\toprule
\textbf{Task} & Question / \textbf{Knowledge} & \textbf{Problem with the knowledge} \\
\midrule
RS & A woman screams. You gointo a shop and find a man lying dead on the floor. There are three people in the room. A postman, a milkman and a doctor. Who killed him? \newline \Right{(A) doctor} (B) police station (C) liars (D) radio (E) water fountain \newline \textbf{The doctor is the one who killed the man.} & \textbf{Ethical risk} \newline This knowledge might impress bias towards a certain profession. However, the question itself should probably take the blame, because unfortunately, "doctor" is the only valid choice given the question's context. \\
\midrule
PIQA & crossing out \newline (A) ugly people from the bachelor is cool \Right{(B) ugly people from planet earth is cool} \newline \textbf{Crossing out ugly people from planet earth is cool.} & \textbf{Ethical risk} \newline This knowledge might impress bias towards a group with certain physical characteristic. \\
\midrule
CSQA & With the card slot lit up he knew how to get started finding his balance with what? \newline (A) slot machine (B) ticket machine (C) bank machine (D) telephone \Right{(E) automated teller} \newline \textbf{A slot machine is a machine that takes cards and uses them to make money.} & \textbf{Ethical risk} \newline This knowledge might advocate for gambling. \\
\bottomrule
\end{tabular}
\caption{
    Examples of knowledge generated by \methodname{} that have potential ethical risks.
}
\label{tab:qual_ethics}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/qual_semantic.tex <==
\begin{table*}[h!]
\setlength{\tabcolsep}{3pt}
\footnotesize
\centering
\begin{tabular}{cp{200pt} p{144pt}}
\toprule
\textbf{Task} & Question / \textbf{Knowledge} & \textbf{Problem with the knowledge} \\
\midrule
RS & I am a fruit. I am tasty and provide lots of energy. You can also find me in a calendar. What am I? \newline (A) shop (B) choppers \Right{(C) date} (D) european (E) movie \newline \textbf{The fruit of the year is the date.} & \textbf{Ambiguous} \newline The knowledge does not specify which year, so it is not possible to verify its factuality. \\
% \midrule
% QuaRTz & Sarah puts two pieces of candy into water. The piece that will break down the fastest is the one that is \newline (A) larger \Right{(B) smaller} & \textbf{Ambiguous} \newline It is ambiguous about what the "piece" is. A smaller piece of candy would break down faster when dissolved in water, whereas a smaller piece of rock would break down slower during weathering. \\
% \midrule
% PIQA & Prepare clay for a kiln \newline \Right{(A) Allow clay to dry completely then take a damp smooth sponge and smooth away imperfections} (B) Soak clay in water then take a damp smooth sponge and smooth away imperfections \newline \textbf{Clay is best prepared by allowing it to dry completely.} & \textbf{Under-specified} \newline The best way to prepare clay may be different for different purposes. The knowledge does not specify the particular purpose (which, however, can arguably be inferred from the question context). \\
\midrule
QuaRTz & Carla is pushing two carts down a street. One cart is heavy, the other is light. The heavy cart, compared to the light one, will accelerate \newline \Right{(A) slowly} (B) quickly \newline \textbf{The heavy cart will accelerate slower than the light one.} & \textbf{Under-specified} \newline Missing the control factor that the forces exerted on the carts are the same. Though this flaw also exists in the question itself. \\
\midrule
RS & What has a head at night but not in the morning? \newline (A) sleeping \Right{(B) pillow} (C) neck (D) shampoo (E) beer \newline \textbf{Sleeping animals have a head at night.} & \textbf{Over-specified} \newline It would be normal to say "animals have a head". It is weird to qualify with "sleeping" and "at night". \\
% \midrule
% QASC & what are all aquatic? \newline (A) insects (B) lizards (C) weater (D) paramecium \Right{(E) jellyfish} (F) angiosperm (G) humans (H) snakes \newline \textbf{Aquatic organisms are all animals that swim.} & \textbf{Over-confident} \newline The use of quantifier "all" is too absolute. Not all animals that swim are aquatic (e.g. swans). An appropriate knowledge could be, \textit{Aquatic animals are animals that swim.} \skyler{I think this knowledge is actually okay - it is saying of the set of aquatic organisms, all of them are animals that can swim. It is like saying ``Cars are all vehicles that move fast''.} \gary{Oh yeah, agreed.} \\
% \midrule
% WG & Kevin ate large amounts of food but not Adam. \_ didn't have to get checked to see if they had a tapeworm. \newline (A) Kevin \Right{(B) Adam} \newline \textbf{Adam didn't have a tapeworm.} & \textbf{Over-confident} \newline It would be appropriate to say the risk that Adam has tapeworm is relatively low. This knowledge is a strech. \\
\midrule
WG & Because William developed a sore knee during his race against against Kyle, \_ won the race. \newline (A) William \Right{(B) Kyle} \newline \textbf{William was not able to run the race.} & \textbf{Over-confident} \newline William might still be able to finish the race with a sore knee. \\
\midrule
RS & what is the begining of enternity the end of life the end of time and the end to every race \newline \Right{(A) e} (B) quick (C) finality (D) fix (E) habit \newline \textbf{The end of every race is the end of every race.} & \textbf{Tautological} \newline This knowledge does not give any meaningful information. \\
\midrule
QuaRTz & Sharon is conducting an experiment on valence electrons and soon discovers that when they are closer to the nucleus, they are \_\_\_\_\_ easily removed from the atom. \newline (A) more \Right{(B) less} \newline \textbf{Valence electrons are more prone to being removed from the atom.} & \textbf{Not applicable} \newline This knowledge implicitly compares the removability of valence vs. non-valence electrons. However, the question needs a comparison of valence electrons in atoms of different sizes, so the knowledge cannot be applied to answering this question. \\
\bottomrule
\end{tabular}
\caption{
    Examples of knowledge generated by \methodname{} which are semantically problematic.
}
\label{tab:qual_sematic}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/qual_social.tex <==
\begin{table*}[h!]
\setlength{\tabcolsep}{3pt}
\footnotesize
\centering
\begin{tabular}{cp{200pt} p{144pt}}
\toprule
\textbf{Task} & Question / \textbf{Knowledge} & \textbf{Problem with the knowledge} \\
\midrule
SIQA & Riley broke loose from the house. He thought he would never get out of there. Why did Riley do this? \newline (A) Stay in the house longer \Right{(B) think about his life} (C) go home for a while \newline \textbf{Breaking out of a bad habit is usually a bad idea.} & \textbf{Social value} \newline This knowledge is a generally true statement, so we labeled it as factual. \\
\midrule
SIQA & Tracy heard a faint buzzing noise and immediately ran for her life. How would you describe Tracy? \newline \Right{(A) scared of bees} (B) sad (C) not phased by bees \newline \textbf{One should not be scared of bees.} & \textbf{Social value} \newline It is hard to decide whether this knowledge should be considered factual or not. \\
\midrule
SIQA & Remy gave Skylar's Netflix account password to one of Remy's other friends. How would Skylar feel as a result? \newline (A) like a bad friend (B) excited \Right{(C) used} \newline \textbf{A friend can be used by a friend.} & \textbf{Social value} \newline It is ambiguous whether \textit{can} means \textit{it is possible that ...}, or \textit{ought to}. If it is the latter, then the knowledge is promoting some problematic social value. \\
\midrule
SIQA & Riley was the best of friends with the boy with cancer. What will Riley want to do next? \newline \Right{(A) visit the hospital} (B) shun the friend (C) become friends with the boy with cancer too \newline \textbf{One should visit their sick friend.} & \textbf{Social value} \newline It is generally a kind thing to visit a sick friend. However, it is conceivable that the friend needs to recover in peace or has some infectious disease, which renders a visit inappropriate. \\
\midrule
SIQA & Carson tried to fight Robin last night because Robin hurt Carson a lot. What will Carson want to do next? \newline (A) apologize (B) do nothing \Right{(C) hurt Robin} \newline \textbf{One should apologize when they hurt someone.} & \textbf{Social value} \newline This knowledge is generally accepted. However, there are extenuating circumstances where hurting someone does not need an apology (e.g. hurting a violent criminal to protect oneself). \\
\midrule
SIQA & Bailey told Alex to send the pdf because they didn't want to do it themselves. How would Alex feel as a result? \newline (A) lazy about work (B) happy \Right{(C) angry} \newline \textbf{One should be willing to help others.} & \textbf{Social value} \newline This knowledge is generally accepted, but it is not a good fit to the question's context. It is normal to be emotional when being ordered to do something on other's behalf. \\
\midrule
SIQA & Kendall wrapped a bandage around my neck after getting injured in a fight. What will Kendall want to do next? \newline (A) harm them (B) punish them \Right{(C) protect them} \newline \textbf{One should help others in need.} & \textbf{Social value} \newline This knowledge is generally accepted, and appropriate to the question's context. \\
\bottomrule
\end{tabular}
\caption{
    Examples of knowledge generated by \methodname{} that express some social value.
}
\label{tab:qual_social}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/rainier.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/rainier_new.png}
\caption{
    \methodname{} can introspect for commonsense knowledge that underpin the reasoning process, and is trained via reinforcement learning, where the reward is derived from the effectiveness of knowledge when prompting a frozen, generic QA model.
}
\label{fig:rainier}
\vspace{-16pt}
\end{figure}

==> [EMNLP 2022] cc-GKM/floats/results.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
% \begin{small}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l cc cc cc cc cc cc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multicolumn{2}{c}{CSQA} & \multicolumn{2}{c}{QASC} & \multicolumn{2}{c}{PIQA} & \multicolumn{2}{c}{SIQA} & \multicolumn{2}{c}{WG} & \multicolumn{2}{c}{\textbf{Avg.}} \\
\textbf{Method} $\downarrow$ & \small{dev} & \small{test} & \small{dev} & \small{test} & \small{dev} & \small{test} & \small{dev} & \small{test} & \small{dev} & \small{test} & \small{dev} & \small{test} \\
\midrule
UQA-large (0.77B) & 61.43 & 53.00 & 43.09 & 45.65 & 63.66 & 65.50 & 53.84 & 57.21 & 53.35 & 54.67 & 55.07 & 55.21 \\
\quad + Few-shot GPT-3-Curie (13B) & 66.34 & -- & 53.24 & -- & 64.25 & -- & \textbf{58.29} & -- & 55.56 & -- & 59.54 & -- \\
\quad + Self-talk GPT-3-Curie (13B) & 63.31 & -- & 49.89 & -- & 65.23 & -- & 51.89 & -- & 52.96 & -- & 56.66 & -- \\
\quad + DREAM (11B) & 64.54 & -- & 49.46 & -- & 64.74 & -- & 51.59 & -- & 56.12 & -- & 57.29 & -- \\
\midrule
\quad \textbf{+ \methodname{}-large (0.77B) [ours]} & \textbf{67.24} & \textbf{60.18} & \textbf{54.97} & \textbf{54.13} & \textbf{65.67} & \textbf{67.09} & 57.01 & \textbf{59.01} & \textbf{56.91} & \textbf{57.39} & \textbf{60.36} & \textbf{59.56} \\
\bottomrule
\end{tabular}
}%
% \end{small}
\vspace{-4pt}
\caption{
    Results on \textbf{seen} datasets.
    All experiments use UnifiedQA-large as the QA model, and optionally uses knowledge from one of the knowledge generation models.
    Skipped baselines are marked with ``--''.
}
\label{tab:results_id}
%
\vspace{16pt}
%
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l cc cc cc cc cc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multicolumn{2}{c}{NS} & \multicolumn{2}{c}{RS} & \multicolumn{2}{c}{QuaRTz} & \multicolumn{2}{c}{HS} & \multicolumn{2}{c}{\textbf{Avg.}} \\
\textbf{Method} $\downarrow$ & \small{dev} & \small{test-all} & \small{dev} & \small{test} & \small{dev} & \small{test} & \small{dev} & \small{test} & \small{dev} & \small{test} \\
\midrule
UQA-large (0.77B) & 26.50 & 19.61 & 28.11 & 38.34 & 68.75 & 67.60 & 35.00 & 34.30 & 39.59 & 41.85 \\
\quad + Few-shot GPT-3-Curie (13B) & 38.00 & -- & 35.65 & -- & 69.01 & -- & 37.33 & -- & 45.00 & -- \\
\midrule
\quad \textbf{+ \methodname{}-large (0.77B) [ours]} & 30.00 & 21.81 & 30.07 & 41.22 & 70.31 & 68.24 & 35.73 & 34.80 & 41.53 & 43.76 \\
\bottomrule
\end{tabular}
}%
\vspace{-4pt}
\caption{
    Results on \textbf{unseen} datasets.
}
\label{tab:results_ood}
% \vspace{-8pt}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/results_id_nope.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{l c cc cc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{OBQA} & \multicolumn{2}{c}{ARC} & \multicolumn{2}{c}{AI2Science} \\
\textbf{Method} $\downarrow$ &  & \small{easy} & \small{hard} & \small{elem} & \small{mid} \\
\midrule
UQA-large (0.77B) & 70.20 & 69.12 & 55.85 & 69.11 & 64.80 \\
\quad + Few-shot GPT-3-Curie (13B) & 68.80 & 71.05 & 56.52 & 70.73 & 65.60 \\
\midrule
\quad \textbf{+ \methodname{}-large (0.77B) [ours]} & 69.60 & 67.72 & 55.18 & 68.29 & 63.20 \\
\bottomrule
\end{tabular}
}%
\vspace{-4pt}
\caption{
    Results on the other 3 \textbf{seen} datasets.
    All experiments use UnifiedQA-large as the QA model, and optionally uses knowledge from one of the knowledge generation models.
    On these datasets, \methodname{}-generated knowledge does not give an improvement over the vanilla QA baseline.
}
\label{tab:results_id_nope}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/results_qa.tex <==
\begin{figure*}
\begin{minipage}{.48\linewidth}
\centering
\includegraphics[width=\linewidth]{images/results_qa_seen.png}
\end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
\centering
\includegraphics[width=\linewidth]{images/results_qa_unseen.png}
\end{minipage}
\vspace{-4pt}
\caption{
    Effectiveness of \methodname{}-generated knowledge on different QA models.
    Average accuracy on dev sets is reported.
    (Note: results of few-shot GPT-3-Curie on Unicorn-large is missing.)
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{fig:results_qa}
% \vspace{-8pt}
\end{figure*}

==> [EMNLP 2022] cc-GKM/floats/selftalk_templates.tex <==
\begin{table*}[b]
\small
\centering
\begin{tabular}{l l}
\toprule
\textbf{Question Template} & \textbf{Answer Template} \\
\midrule
What is the definition of & The definition of \_ is \\
What is the main purpose of & The purpose of \_ is to \\
What is the main function of a & The main function of a \_ is \\
What are the properties of a & The properties of a \_ are that \\
What is a & \_ is \\
What happened as a result of & As a result of \_, \\
What might have caused & The cause of \_ was \\
What is a part of & A part of \_ is \\
What is an example of & An example of \_ is \\
How would you & One would \_ by \\
\bottomrule
\end{tabular}
\caption{Templates used in the self-talk baseline.}
\label{tab:selftalk_templates}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/trash/human_cats.tex <==
\begin{table*}
\centering
\resizebox{0.75 \textwidth}{!}{%
\begin{tabular}{lrrrrrrrrr}
\toprule
& CSQA & QASC & PIQA & SIQA & WG & NS & RS & QuaRTz & \textbf{All} \\
\midrule
\textbf{Domains} \\
scientific & 13\% & 79\% & 6\% & 0\% & 0\% & 20\% & 21\% & 84\% & 25\% \\
social & 24\% & 0\% & 6\% & 94\% & 59\% & 10\% & 9\% & 0\% & 27\% \\
physical & 34\% & 10\% & 11\% & 0\% & 4\% & 0\% & 3\% & 21\% & 12\% \\
temporal & 5\% & 14\% & 0\% & 3\% & 4\% & 0\% & 0\% & 0\% & 4\% \\
numerical & 0\% & 0\% & 3\% & 0\% & 0\% & 90\% & 3\% & 5\% & 5\% \\
\midrule
\textbf{Relations} \\
definition & 5\% & 3\% & 0\% & 0\% & 0\% & 0\% & 35\% & 5\% & 7\% \\
attribute & 39\% & 62\% & 28\% & 39\% & 74\% & 60\% & 32\% & 53\% & 46\% \\
part of & 3\% & 7\% & 3\% & 0\% & 0\% & 30\% & 12\% & 0\% & 5\% \\
member of & 3\% & 7\% & 0\% & 0\% & 0\% & 10\% & 12\% & 0\% & 4\% \\
capable of & 5\% & 7\% & 28\% & 3\% & 0\% & 0\% & 3\% & 5\% & 8\% \\
purpose & 0\% & 7\% & 28\% & 0\% & 0\% & 0\% & 6\% & 5\% & 7\% \\
causality & 3\% & 10\% & 3\% & 0\% & 0\% & 0\% & 0\% & 16\% & 4\% \\
strategy & 11\% & 10\% & 22\% & 3\% & 0\% & 0\% & 0\% & 0\% & 7\% \\
\midrule
\textbf{Syntax} \\
negation & 3\% & 0\% & 6\% & 10\% & 19\% & 10\% & 18\% & 0\% & 8\% \\
comparison & 8\% & 7\% & 17\% & 3\% & 30\% & 0\% & 0\% & 79\% & 16\% \\
condition & 5\% & 0\% & 8\% & 0\% & 0\% & 0\% & 0\% & 11\% & 3\% \\
because & 11\% & 0\% & 3\% & 0\% & 7\% & 0\% & 0\% & 0\% & 3\% \\
\bottomrule
\end{tabular}
}%
\caption{
    Percentage of \methodname{}-generated knowledge categorized by domain, expressed relation, and syntax.
    The percentages do not add up to 100\% because some knowledge have none of these characteristics, while some others may have multiple. \hanna{This table is not readable; first, you don't need all those \%s it just confuses the reader; maybe a bar chart? there are too many numbers here, which makes things harder to read ?or some sort of heatmap?}
    \skyler{I think this would look good as three comparative bar charts: Domain, Relation, and Syntax, so we can see the distribution of each of the datasets}
}
\label{tab:human_cats}
\vspace{-16pt}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/trash/hypers_short.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c c p{138pt}}
\toprule
\textbf{Symbol} & \textbf{Value} & \textbf{Description} \\
\midrule
\multicolumn{3}{c}{\textsc{Training Stage I: Imitation Learning}} \\
\midrule
$M$ & 20 & Number of knowledge statements to sample from GPT-3, per question. \\
$p$ & 0.5 & Parameter for nucleus sampling from GPT-3. \\
% $L_{\text{output}}$ & 64 & Max length of output from GPT-3. \\
% $L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
% $L_{\text{output}}$ & 64 & Max length of output from \methodname{} (i.e. generated knowledge). \\
$B$ & 64 & Batch size for training. \\
$S$ & 50,000 & Total number of training steps. \\
$\eta$ & $1 \times 10^{-5}$ & Learning rate of Adam optimizer. \\
\midrule
\multicolumn{3}{c}{\textsc{Training Stage II: Reinforcement Learning}} \\
\midrule
$\alpha$ & 1.0 & Weight of value model loss in PPO. \\
$\beta$ & 0.2 & Weight of entropy bonus term in reward. \\
$\gamma$ & 1.0 & Discount factor for rewards. \\
$\lambda$ & 0.95 & Parameter for advantage estimation. \\
$\eps$ & 0.2 & Clipping range for the \textit{clipped surrogate objective}. \\
% $L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
% $L_{\text{output}}$ & 32 & Max length of output from \methodname{} (i.e. generated knowledge). \\
$\tau$ & 0.7 & Temperature for knowledge sampling in PPO training. \\
% $E$ & 1M & Total number of training episodes. \\
$B$ & 64 & Batch size for training. \\
$S$ & 15,625 & Total number of training steps. \\
% $s$ & 4 & Interval (in steps) for updating the lagging models (policy and value). \\
$\eta$ & $2 \times 10^{-5}$ & Learning rate of Adam optimizer (with a linear learning rate decay schedule). \\
\midrule
\multicolumn{3}{c}{\textsc{Inference}} \\
\midrule
$M$ & 10 & Number of knowledge statements to sample from \methodname{}, per question. \\
$p$ & 0.5 & Parameter for nucleus sampling from \methodname{}. \\
% $L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
% $L_{\text{output}}$ & 32 & Max length of output from \methodname{}. \\
\bottomrule
\end{tabular}
\caption{
    Hyperparameter settings (partial).
    See \autoref{tab:hypers} for full list.
}
\label{tab:hypers_short}
\vspace{-8pt}
\end{table}

==> [EMNLP 2022] cc-GKM/floats/trash/ppoo.tex <==
\begin{algorithm*}
\small
\caption{Training \methodname{}, Stage II, Reinforcement Learning; \hanna{for this algorithm (you can move it to appendix, but in the main text simplify it a lot; basically you have equations in the text and are repeating it here; Just say Lpolicy calculate through eq. blah blah; LPPo calculate through eq blah blah and remove all the rest of the previous things. you just need to list the big training steps where is the }}
\begin{algorithmic}
\Procedure{ReinforcementLearning}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\phi_0$, $\psi_{\text{QA}}$}
    \Procedure{ComputeRewardNormalizationFactors}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\psi_{\text{QA}}$}
        \State $\mathcal{R}_{\text{init}} \gets \{\}$
        \ForAll {$x = (q, A, a^*) \in \Ds_{\text{ID}}$}
            \State $k \gets$ \Call{TemperatureSampling}{$q$, $\theta_{\text{imit}}$, $\tau$}
            \State $r \gets r(x, k; \psi_{\text{QA}})$
            \State $\mathcal{R}_{\text{init}} \gets \mathcal{R}_{\text{init}} \cup \{ r \}$
        \EndFor
        \State $\mu_0 \gets \mu(\mathcal{R}_{\text{init}})$, $\sigma_0 \gets \sigma(\mathcal{R}_{\text{init}})$
        \State \Return $(\mu_0, \sigma_0)$
    \EndProcedure
    \State $(\mu_0, \sigma_0) \gets$ \Call{ComputeRewardNormalizationFactors}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\psi_{\text{QA}}$}
    \State $\theta \gets \theta_{\text{imit}}$, $\phi \gets \phi_0$
    \State $\theta_{\text{old}} \gets \theta$, $\phi_{\text{old}} \gets \phi$
    \For {$i = 1 \hdots S$}
        \State \textit{batch} $\gets$ sample a batch of size $B$ from $\Ds_{\text{ID}}$
        \State $\mathcal{L}_{\text{Policy}} \gets 0$, $\mathcal{L}_{\text{Value}} \gets 0$
        \ForAll {$(q, A, a^*) \in$ \textit{batch}}
            \State $k \gets$ \Call{TemperatureSampling}{$q$, $\theta$, $\tau$}
            \State $r \gets r(x, k; \psi_{\text{QA}})$
            \State $r \gets (r - \mu_0) / \sigma_0$
            \State $R \gets r - \beta \log{\big( p_K(k | q; \theta) / p_K(k | q; \theta_{\text{imit}}) \big)}$
            \State $T \gets |k|$
            \State $r_T \gets R$, $r_{[1 \hdots T-1]} \gets 0$
            \For {$t = T \hdots 1$}
                \State $\delta_t \gets r_t + \gamma V(s_{t+1}; \phi) - V(s_t; \phi)$
                \State $\hat{A}_t \gets \delta_t + (\gamma \lambda) \delta_{t+1} + \hdots + (\gamma \lambda)^{T-t+1} \delta_{T-1}$
                \State $V_t^{\text{targ}} \gets r_t + \gamma r_{t+1} + \hdots + \gamma^{T-t+1} r_{T-1} + \gamma^{T-t} V(s_T; \phi_{\text{old}})$
                \State $\nu_t \gets p_K(k_t | q; \theta) / p_K(k_t | q; \theta_{\text{old}})$
                \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} - \min \big( \nu_t \hat{A}_t, \text{clip}(\nu_t, 1 - \eps, 1 + \eps) \hat{A}_t \big)$
                \State $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} + (V(s_t; \phi) - V_t^{\text{targ}})^2$
            \EndFor
            \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} / T$, $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} / T$
        \EndFor
        \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} / B$, $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} / B$
        \State $\mathcal{L}_{\text{PPO}} \gets \mathcal{L}_{\text{Policy}} + \alpha \cdot \mathcal{L}_{\text{Value}}$
        \State $\theta \gets \theta - \eta \cdot \nabla_\theta \mathcal{L}_{\text{PPO}}$, $\phi \gets \phi - \eta \cdot \nabla_\phi \mathcal{L}_{\text{PPO}}$
        \If {$i \equiv 0 (\text{mod } s)$} \Comment{Update the lagging policy every $s$ steps.}
            \State $\theta_{\text{old}} \gets \theta$, $\phi_{\text{old}} \gets \phi$
        \EndIf
        \State \Return $\theta$
    \EndFor
\EndProcedure
\end{algorithmic}
\label{alg:ppoo}
\end{algorithm*}

==> [EMNLP 2022] cc-GKM/floats/trash/results.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l ccccccccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{OBQA} & \multicolumn{2}{c}{ARC} & \multicolumn{2}{c}{AI2Science} & \multirow{2}{*}{CSQA} & \multirow{2}{*}{QASC} & \multirow{2}{*}{PIQA} & \multirow{2}{*}{SIQA} & \multirow{2}{*}{WG} & \textbf{Avg.} \\
\textbf{Method} $\downarrow$ &  & \small{easy} & \small{hard} & \small{elem} & \small{mid} & & & & & & (last 5) \\
\midrule
UQA & 70.20 & 69.12 & 55.85 & 69.11 & 64.80 & 61.43 & 43.09 & 63.66 & 53.84 & 53.35 & 55.07 \\
\methodname{} (T5-large) + UQA & 69.60 & 67.72 & 55.18 & 68.29 & 63.20 & \textbf{67.24} & \textbf{54.97} & \textbf{65.67} & \textbf{57.01} & \textbf{56.91} & \textbf{60.36} \\
\midrule
Few-shot GPT-3 (13B) + UQA & 68.80 & 71.05 & 56.52 & 70.73 & 65.60 & 66.34 & 53.24 & 64.25 & 58.29 & 55.56 & 59.54 \\
Self-talk GPT-3 (13B) + UQA & -- & -- & -- & -- & -- & 63.31 & 49.89 & 65.23 & 51.89 & 52.96 & 56.66 \\
DREAM (11B) + UQA & -- & -- & -- & -- & -- & 64.54 & 49.46 & 64.74 & 51.59 & 56.12 & 57.29 \\
\bottomrule
\end{tabular}
}%
\vspace{-6pt}
\caption{
    Results on in-domain datasets.
    Accuracy on dev set is reported.
    Predictions made by UQA-large.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_id}
%
\vspace{6pt}
%
\begin{minipage}[t]{.49 \linewidth}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l cccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{CSQA} & \multirow{2}{*}{QASC} & \multirow{2}{*}{PIQA} & \multirow{2}{*}{SIQA} & \multirow{2}{*}{WG} & \multirow{2}{*}{\textbf{Avg.}} \\
\textbf{Method} $\downarrow$ \\
\midrule
UQA & 53.00 & 45.65 & 65.50 & 57.21 & 54.67 & 55.21 \\
\methodname{} (T5-large) + UQA & \textbf{60.18} & \textbf{54.13} & \textbf{67.09} & \textbf{59.01} & \textbf{57.39} & \textbf{60.00} \\
\bottomrule
\end{tabular}
}%
\vspace{-6pt}
\caption{
    Results on in-domain datasets.
    Accuracy on test set is reported.
    Predictions made by UQA-large.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_id_test}
\end{minipage}
%
\hfill
%
\begin{minipage}[t]{.49 \linewidth}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l cccccccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{NS} & \multirow{2}{*}{RS} & \multirow{2}{*}{QuaRTz} & \multirow{2}{*}{HS} & \multirow{2}{*}{\textbf{Avg.}} \\
\textbf{Method} $\downarrow$ \\
\midrule
UQA & 26.50 & 28.11 & 68.75 & 35.00 & 39.59 \\
\methodname{} (T5-large) + UQA & \textbf{30.00} & \textbf{30.07} & \textbf{70.31} & \textbf{35.73} & \textbf{41.53} \\
\midrule
Few-shot GPT-3 (13B) + UQA & 38.00 & 35.65 & 69.01 & 37.33 & 45.00 \\
\bottomrule
\end{tabular}
}%
\vspace{-6pt}
\caption{
    Results on out-of-domain datasets.
    Accuracy on dev set is reported.
    Predictions made by UQA-large.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_ood}
\end{minipage}
%
\vspace{12pt}
%
\centering
\resizebox{0.8 \textwidth}{!}{%
\begin{tabular}{l cccccccccccc}
\toprule
\textbf{QA Model} $\rightarrow$ & \multicolumn{2}{c}{UQA-small} & \multicolumn{2}{c}{UQA-base} & \multicolumn{2}{c}{UQA-large} & \multicolumn{2}{c}{UQA-3b} & \multicolumn{2}{c}{Unicorn-large} \\
\textbf{Knowledge Gen.} $\downarrow$ & ID & OOD & ID & OOD & ID & OOD & ID & OOD & ID & OOD \\
\midrule
None & 39.07 & 25.51 & 45.51 & 31.19 & 55.07 & 39.59 & 66.51 & 43.72 & 50.80 & 39.94 \\
\methodname{} (T5-large) & \textbf{48.60} & \textbf{27.99} & \textbf{54.77} & \textbf{37.21} & \textbf{60.36} & \textbf{41.53} & \textbf{67.85} & \textbf{45.45} & \textbf{59.86} & \textbf{41.90} \\
\quad $\Delta$ & \;+9.53 & \;+2.48 & \;+9.26 & \;+6.02 & \;+5.29 & \;+1.94 & \;+1.34 & \;+1.73 & \;+9.06 & \;+1.96 \\
\midrule
Few-shot GPT-3 (13B) & 46.88 & 28.68 & 52.80 & 43.17 & 59.54 & 45.00 & 67.42 & 52.23 & -- & -- \\
\bottomrule
\end{tabular}
}%
\vspace{-6pt}
\caption{
    Effectiveness of generated knowledge on different QA models.
    Average accuracy on dev set is reported.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_qa}
\vspace{-8pt}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/trash/results_ood.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{0.8 \textwidth}{!}{%
\begin{tabular}{l cccccccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{NumerSense} & \multirow{2}{*}{RiddleSense} & \multirow{2}{*}{QuaRTz} & \multirow{2}{*}{HellaSwag} & \multirow{2}{*}{\textbf{Avg.}} \\
\textbf{Knowledge Gen.} $\downarrow$ \\
\midrule
None & 26.50 & 28.11 & 68.75 & 35.00 & 39.59 \\
\methodname{} (T5-large) & \textbf{30.00} & \textbf{30.07} & \textbf{70.31} & \textbf{35.73} & \textbf{41.53} \\
\bottomrule
\end{tabular}
}%
\vspace{2pt}
\caption{
    Results on out-of-domain datasets.
    Accuracy on dev set is reported.
    Predictions made by UnifiedQA-large.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_ood}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/trash/results_qa.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{0.66 \textwidth}{!}{%
\begin{tabular}{l cccccccccc}
\toprule
\textbf{QA Model} $\rightarrow$ & \multicolumn{2}{c}{UQA-small} & \multicolumn{2}{c}{UQA-base} & \multicolumn{2}{c}{UQA-large} & \multicolumn{2}{c}{UQA-3b} \\
\textbf{Knowledge Gen.} $\downarrow$ & ID & OOD & ID & OOD & ID & OOD & ID & OOD \\
\midrule
None & 39.07 & 25.51 & 45.51 & 31.19 & 55.07 & 39.59 & 66.51 & 43.72 \\
\methodname{} (T5-large) & \textbf{48.60} & \textbf{27.99} & \textbf{54.77} & \textbf{37.21} & \textbf{60.36} & \textbf{41.53} & \textbf{67.85} & \textbf{45.45} \\
\midrule
$\Delta$ & +9.53 & +2.48 & +9.26 & +6.02 & +5.29 & +1.94 & +1.34 & +1.73 \\
\bottomrule
\end{tabular}
}%
\vspace{-4pt}
\caption{
    Effectiveness of generated knowledge on different QA models.
    Average accuracy on dev set is reported.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_qa}
\end{table*}

==> [EMNLP 2022] cc-GKM/floats/uniknower.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/uniknower.png}
\caption{
    \gary{TODO: Redo this figure.}
    \methodname{} can generate relevant knowledge that grounds the reasoning process for commonsense questions in a wide range of domains.
}
\label{fig:uniknower}
\vspace{-16pt}
\end{figure}

==> [EMNLP 2022] cc-GKM/sections/ack.tex <==
\section*{Acknowledgements}
% I would like to thank Ximing Lu, Skyler Hallinan, and Pengfei He for collaborating on this research project.
% Also thanks to my advisors Yejin Choi and Hannaneh Hajishirzi for their valuable feedback.
%
This work was funded in part by the DARPA MCS program through NIWC Pacific (N66001-19-2-4031), NSF IIS-2044660, and ONR N00014-18-1-2826.
We thank OpenAI for offering access to the GPT-3 API.

We would like to thank Prithviraj Ammanabrolu, Alisa Liu and Weijia Shi for the discussion and feedback on early drafts of the paper.
We also thank the anonymous reviewers for their valuable feedback.

==> [EMNLP 2022] cc-GKM/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\input{floats/qual}

\dif{
We introduced \methodname{}, a neural model that can introspect for relevant knowledge on a broad range of commonsense question answering tasks.
% We showed the importance of both of our proposed training stages, imitation learning followed by reinforcement learning, and also showed how we chose a good reward function for model training. \yejin{the second sentences reads a bit awkward to me, perhaps because it's emphasizing the importance of *both* our proposed stages without first explaining the big picture just yet --- explaining them in the remainder of the sentence is a bit strange way of crafting the summary take-away sentences for conclusions. also this sentence comes across to me as a bit too low-level or not exciting...}
\methodname{} is trained with a novel adaption of reinforcement learning, and does not need gold knowledge labels that are difficult to obtain.
Knowledge generated by \methodname{} can serve as useful prompts that improves the performance of QA models on both seen and unseen benchmarks, and outperform knowledge elicited from a few-shot GPT-3 which is 16x bigger.
\methodname{} generates knowledge in the form of natural language statements that are fluent, meaningful, high-quality, and diverse in terms of domain and relation; furthermore, the effect of these knowledge on the QA model is found to align well with human judgments.
}

% In future work, we would like to extend \methodname{} so that it supports multi-step knowledge introspection, i.e. chaining multiple knowledge statements in each reasoning path.
% Additionally, we would like to explore better knowledge integration methods that adaptively fit to the required depth of reasoning.
% Through these extensions, we hope to yield a more systematic view of commonsense reasoning via the lens of knowledge introspection.

==> [EMNLP 2022] cc-GKM/sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

% \input{floats/hypers_short}

\paragraph{Seen datasets.}
For both imitation learning and reinforcement learning, we use the 8 multiple-choice datasets that $\text{UnifiedQA}_{\text{v2}}$ \citep{khashabi2022unifiedqa} uses for training:
OpenBookQA \citep{mihaylov2018can}, ARC \citep{clark2018think}, AI2Science \citep{clark2018think}, CommonsenseQA \citep{talmor2018commonsenseqa}, QASC \citep{khot2020qasc}, PhysicalIQA \citep{bisk2020piqa}, SocialIQA \citep{sap2019socialiqa}, and Winogrande \citep{sakaguchi2021winogrande}.\footnote{We exclude MCTest and RACE because most questions in these reading comprehension datasets are too long to fit into our model's input.}

\paragraph{Unseen datasets.}
We additionally evaluate our method on the following 4 multiple-choice QA datasets that our model was \textit{not} trained on:
NumerSense \citep{lin2020birds}, RiddleSense \citep{lin2021riddlesense}, QuaRTz \citep{tafjord2019quartz}, and HellaSwag \citep{zellers2019hellaswag}.

\paragraph{Models.}
For Stage I training, we get silver knowledge from the GPT-3-Curie (13B) model \citep{brown2020language}.
The knowledge introspector is initialized with T5-large \citep{raffel2019exploring}, which has 0.77B parameters.
For Stage II training, we initialize the value model with T5-large, and replace the language modeling head with a value regression head, which is initialized from scratch; we use UnifiedQA-large (UQA-large) \citep{khashabi2020unifiedqa} as the QA model that provides reward, which means the text concatenation function is defined as $q \circ k =$ \texttt{\{q\} \textbackslash{}n \{k\}}.
We use the same question formatting as UnifiedQA.
See \autoref{tab:hypers} for hyperparameters.

% \hanna{i was lost on what datasets you have the GPT3 demonstrations. }
% \paragraph{Hyperparameters.}
% See \autoref{tab:hypers}.
% We truncate the model inputs to no more than 256 tokens, and the model outputs to no more than 32 tokens, except for Stage I training where we did 64 tokens.

\paragraph{Baselines.}
We mainly report performance improvements over the vanilla QA baseline (i.e. direct inference with the UnifiedQA-large model and without prompting \methodname{}-generated knowledge).
We also consider using knowledge from:
\begin{itemize}
\item Few-shot GPT-3 \citep{liu2021generated}, where knowledge statements are elicited from the GPT-3-Curie (13B) model -- under the same prompts used for getting silver knowledge in Stage I training (\S\ref{sec:method_imit}), and the same hyperparameter setting for decoding ($M = 10$ knowledge per question, with nucleus sampling where $p = 0.5$).
\item Self-talk \citep{shwartz2020unsupervised}, where we generate $M = 10$ knowledge per question with GPT-3-Curie and a variety of templates.
\item DREAM \citep{gu2021dream}, where we generate $M = 10$ scene elaborations per question with the DREAM (11B) model.
\end{itemize}
See \S\ref{sec:baselines} for more details on these baselines.
We do not compare with chain-of-thought prompting \citep{wei2022chain} because it relies on emergent behaviors that does not exist in the scale that we experiment with.


==> [EMNLP 2022] cc-GKM/sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\input{floats/rainier}

% \hanna{1. previous work (including yours) has also shown that generated knowledge is helpful. you need to refer to that and say they are domain specific blah blah; you need to contrast important features of your work with previous approraches.
% 2. you argue for RL since it is discrete; I don't buy that argument. 
% 3. why do you argue for frozen inference model? }

\dif{
Commonsense is a significant challenge for modern NLP models, due to the obscurity of underlying knowledge that grounds the reasoning process.
% \yejin{this opening sentence is excellent! crisp and attention grabbing}
While humans are generally able to \textit{introspect} the underlying reasons for their conclusion \citep{Mercier2017TheEO},
% \yejin{bibtex bug? the 2nd author sperber is missing. also, it's a stretch to say that (the book claims that) humans are correctly aware of the unconscious reasons}
neural models
% usually make direct, intuitive-ish \yejin{LOL '-ish' in a paper is too casual...} inferences and
lack the capability to verbalize the premises leading to their prediction.
% \yejin{``neural models usually make direct, intuitive inferences'` also reads as  an ungrounded and hand-wavy claim; we can rephrase this whole sentence to avoid the unnecessary and ungrounded (or even incorrect) claims, e.g., ``while humans can introspect and provide plausible reasons underlying their decisions, neural QA models  lack such capability to verbalize...''  (providing is different from being correctly aware)}
This hinders models' performance and robustness on commonsense tasks, and makes it difficult to inspect their point of failure.
Recent research has demonstrated that relevant knowledge can provide useful context for approaching commonsense tasks.
Yet these methods either retrieve from in-domain knowledge bases \cite{mitra2019additional, chang2021incorporating} that do not have good coverage over commonsense, or generate knowledge from neural models \citep{shwartz2020unsupervised, gu2021dream, liu2021generated}, which often need domain-specific engineering and very large models (e.g. GPT-3 \citep{brown2020language}).
It is still an open challenge to systematically find high-quality knowledge.
% but these models often require manual interventions on task-specific data or rely on very large models (e.g. GPT-3~\cite{brown2020language}). 

In this work, we \dif{use} a novel, reinforcement-learning-based method to develop \methodname{}, a generative neural model that can introspect the underlying knowledge for reasoning about commonsense questions. As illustrated in Fig \ref{fig:rainier}, \methodname{} is trained to  generate knowledge that are both fluent natural language statements, and  useful \textit{prompts} that optimize the performance of a generic question answering (QA) model. 
Our model (1) demonstrates strong generalization to unseen benchmarks \dif{without additional engineering effort (e.g. finetuning)},
% \yejin{too informal... how about `without additional finetuning'} \gary{`finetuning' won't cover all, since some are template design. How about `without additional engineering effort'}
(2) \dif{produces commonsense knowledge of high quality and diversity,}
% \yejin{broad coverage across diverse commonsense reasoning benchmarks; it's a tad imprecise to say broad coverage of commonsense knowledge, as this paper won't be evaluated for a broad coverage commonsense KB} \gary{I agree, since we don't evaluate for completeness. But `across diverse commonsense benchmarks' is bit repetitive to (1). I guess `quality and diversity' can be a tone down compared to `coverage'.}
and (3) \dif{is substantially smaller in size compared to GPT-3, the best knowledge source reported so far.}
% \yejin{just stating `moderate size' reads too vague (why does the size matter suddenly? moderate w.r.t. what?); we can instead say, ``substantially smaller in size compared to GPT-3, which is the best knowledge source reported in the prior work'' to better contextualize why we are talking about the size...}
%In particular, we show  the benefit of incorporating the generated knowledge to a question answering model, even if they are not directly trained to integrate such knowledge. if high quality knowledge is provided as additional context, even SOTA models that are not trained to integrate such knowledge has been shown to benefit considerably

%power of knowledge. In particular, if high quality knowledge is provided as additional context, even SOTA models that are not trained to integrate such knowledge has been shown to benefit considerably…Recent research demonstrates that relevant knowledge can provide useful context for commonsense tasks \citep{gu2021dream, liu2021generated}, yet it is an open challenge to systematically find knowledge that is of high quality.
}

% \yejin{(1) one of the key theses of the enigma of reason is the tight interplay between reasoning and communication in language, especially that reasoning serves the goal of justifying one's decisions in the eyes of others... that angle is something we could make a connection to in this paper, that our approach maybe be viewed as a computational take on justifying an answer to a question via natural language reasons
% }

% \yejin{(2) another potentially relevant paper to cite about the tight connection between knowledge and reasoning is "The Curious Case of Commonsense Intellgience'' for the Daedalus's special issue on AI & Society, in which i argue that they are in the continuum}

% \gary{TODO: Rework the first paragraph. Find a better quote from psychology.}
% Commonsense is a significant challenge for modern NLP models.
% When making commonsense inferences, the underlying knowledge that grounds the reasoning process is often implicit.
% While humans can deliberately convert from the "fast thinking" mode to "slow thinking" \citep{kahneman2011thinking} by \textit{introspecting} the knowledge under their reasoning process, machines in general lack the capability to verbalize the relevant premises that lead to their conclusion.
% This hinders machine's performance on commonsense tasks and makes it difficult to inspect the model's point of failure.

% \input{floats/uniknower}

% \hanna{I have commented out the following, just make sure that you don't forget to cite them.}
%These make our approach stand out from prior work that generate intermediate text artifacts that facilitate the reasoning process \citep{shwartz2020unsupervised, gu2021dream, paranjape2021prompting, liu2021generated}, which often need heavy engineering on domain-specific data, have weak out-of-domain generalization, and sometimes rely on very large models (e.g. GPT-3).
%Our approach also contrasts with methods that retrieve from in-domain knowledge bases \citep{mitra2019additional, chang2021incorporating}, which do not have good coverage over commonsense.

% Some prior work proposed to alleviate this problem by retrieving knowledge from in-domain knowledge bases \citep{mitra2019additional, chang2021incorporating}, yet arguably even the union of existing knowledge bases 
% % (e.g. ConceptNet \citep{speer2017conceptnet}, ATOMIC \citep{sap2019atomic}, WikiHow \citep{koupaee2018wikihow})
% is not sufficient to cover the wide spectrum of human commonsense.
% Others propose to generate intermediate text artifacts (e.g. explanations \citep{rajani2019explain, latcinnik2020explaining, paranjape2021prompting}, elaborations \citep{shwartz2020unsupervised, gu2021dream}, knowledge paths \citep{bansal2021cose}) that facilitate the reasoning process, but these methods are often heavily engineered on domain-specific data and thus do not have good out-of-domain generalization.
% \cite{liu2021generated} uses few-shot GPT-3 to generate relevant knowledge, yet its dependency on very large models and manually-written, domain-specific demonstrations hinders its usability.

% In this work, we develop \methodname{}, a generative language model that can \textit{introspect} the relevant knowledge underlying a given commonsense question.
% This model is trained on a variety of commonsense datasets, and is shown to possess strong generalization on handling questions from domains it has not seen during training.
% % It is thus a unified knowledge generator that can generate relevant knowledge for questions in arbitrary commonsense domains.
% \methodname{} generates knowledge statements in the form of free text, allowing for more flexibility on the nature of the knowledge compared with prior work, and can be conveniently used to prompt most neural NLP models.
% Compared with \cite{liu2021generated}, our model is much smaller and does not need domain-specific prompts in order to work.


% Meanwhile, we keep the QA model fixed so as to encourage the knowledge to be generically useful for prompting QA models, not just targeting one QA model that is trained to fit \methodname{}. % so it is not tailored to adapt to the knowledge generator.
% \yejin{the previous sentence requires revision; the point isn't compelling or crisp enough. perhaps we could say that ``In order to ensure that RAINIER learns to generate relevant knowledge for a broad range of QA models, we train only the knowledge generator part without fine-tuning the QA model itself to a specific QA dataset''}
\dif{To train \methodname{}, we optimize knowledge introspection for the resulting QA, instead of direct supervision, because there are usually no gold knowledge labels on commonsense datasets.}
% \yejin{we can not refer the previous point by (2)... this reads either too informal or too rough}
\dif{In order to ensure that our model learns to generate generically useful knowledge for a broad range of QA models, we train only \methodname{}, the knowledge introspector, without finetuning the QA model.}
Since our desired knowledge are sequences of discrete, non-differentiable word tokens, we adapt a reinforcement learning algorithm, Proximal Policy Optimization (PPO) \citep{schulman2017proximal, ouyang2022training}, to optimize the knowledge introspector.
Specifically, the reward is defined as the effect of \methodname{}-generated knowledge on the QA model's prediction.
We train \methodname{} in a multi-task setting on 8 commonsense QA datasets -- encompassing general, scientific, physical, and social commonsense -- to equip the model with better generalization to unseen benchmarks.

Experiments show that \methodname{} substantially improves the performance of QA models on 9 commonsense benchmarks (5 datasets seen during training and 4 unseen datasets), and gives larger and more consistent gains than a few-shot GPT-3 \citep{liu2021generated} despite being 16x smaller in parameter size.
It also boosts the performance on top of those QA models that it is not trained against, indicating that it generates generically useful knowledge instead of merely hacking into the reward given by a single QA model.
Knowledge generated by \methodname{} can even boost a QA model that is 4x larger than it, showing the promise of using model-generated knowledge as a complement to model scaling in making progress in commonsense reasoning.
Our analyses show that the knowledge generated by \methodname{} are of high quality, and are diverse in terms of domain (e.g. scientific, social), relation expressed (e.g. part of, member of, purpose), and syntactic property (e.g. negation, comparison).
The effect of these knowledge on the QA model also aligns well with human judgments.
The success of \methodname{} shows that moderately-sized models can serve as source of high-quality and useful commonsense knowledge that facilitates reasoning.
We publicly release the code, the trained \methodname{} model, and the commonsense datasets extended with knowledge generated by \methodname{}.


==> [EMNLP 2022] cc-GKM/sections/limitations.tex <==
\section*{Limitations}
\label{sec:limitations}

\dif{
Despite the positive effect of our knowledge introspector \methodname{} on commonsense QA tasks,
% \yejin{calling our model having an `incredible capability' will do more harms to ourselves than good in the eyes of reviewers...}
its performance on non-commonsense applications is unknown and thus requires further investigation.
Even for commonsense applications, there is still a large gap between model performance and human performance, so the resulting model is not ready for real-world applications.
}
% \yejin{I don't think it is a correct conclusion to state that our method should be only used for commmonsense applications; instead, we should say that performances on non-commonsense applications are unkonwn, thus requires further investigation; even for commonsense applications, there's a large gap between the model performance and human performance, thus the resulting model isn't ready for real world applications...}
% It is unknown how well it can generate factoid knowledge (e.g. the hometown of a celebrity).
There is also a limit on the length of knowledge it generates in our experimental setting, and it has not been tested on generating long and coherent text.
Furthermore, in some cases it may generate knowledge that express inappropriate social values (\autoref{tab:qual_social}), are culture-specific (\autoref{tab:qual_culture}), or contain ethical risks (\autoref{tab:qual_ethics}).
See \S\ref{sec:analysis_more} for examples.
Extra care should be taken when applying our model in production environments, especially when making critical decisions or exposing its generated contents directly to human end users.


==> [EMNLP 2022] cc-GKM/sections/method.tex <==
\section{Method}
\label{sec:method}

% \hanna{you need to reverse the order of your explanations.... when you say knowledge generator, it is not clear right in the first sentence, generating the knowledge for what? you need an overview paragraph or subsection here; in the overview; you first want to define the problem;  say you want to answer a multiple choice question commonsense question; this work focuses on a knowledge generator  define the problem that a commonsense QA tasks is a question + multiple choice. then you need a quick overview that a model consists of a generator + inference, then you focus on generator. Also, talk about your evaluation modes of in-domain vs. out-of-domain more concretely especially if you are highlighting the property of your model that can be generalized to other domains,  }

% \hanna{There are different settings that I lost track of: 
% 1. in-domain data -> I think they are called in-domain because your inference model unifiedQA has seen those data points in training. out-of-domain -> your inference model hasn't seen them. Then, for imitation learning you are using domain-specific demonstrations to generate GPT3 knowledge statements. Are you doing it for all datasets? just in-domain? }


% \hanna{add paragraph headers to organize the section, something like what I am adding below. }

\paragraph{Problem Overview.}
% \hanna{here, you define the problem, and that you want to have a Qa model + knowledge generator, but the challenge is knowledge generator does not have labeled data.}
We focus on the tasks of multiple-choice commonsense QA, consisting of instances of format $x = (q, A, a^*)$, where $q$ is the question, $A$ is the set of candidate answers, and $a^* \in A$ is the correct answer.
For full contextualization, we append candidate answers $A$ to the question $q$ to form the input to the QA model as follows:
% \dif{For full contextualization, we transform the question $q$ so it also contains a serialized version of the candidate answer set $A$, i.e.,}
\begin{align*}
q = \texttt{\small \{question\} (A) \{choice\_A\} (B) \{choice\_B\} ...}
\end{align*}
% \yejin{it's fine to include all the candidate answers in q, but this then becomes redundant with A defined above, which was also the set of candidate answers, which gives out a clunky impression...}
% Our goal is to improve the performance of QA models on these tasks. \hanna{Complementary to commons approaches, right? because we use an underlying QA model as well? Maybe write it this way: common approaches only train QA. To complement... }
Common approaches only train supervised QA models.
As a complement,
% In contrast to common approaches that train the QA models, 
we train a separate model, which we refer to as \methodname{}, that can introspect question-specific knowledges
% \hanna{introspect knowledge given a LM?}
that are useful to \textit{prompt} a fixed QA model.
\methodname{} is a sequence-to-sequence language model, $p_K(k | q; \theta)$, and we expect it to generate knowledge statements ($k$'s) in response to the given question ($q$).
% \ximing{how about: We expect \methodname{} to generate knowledge statements $k$'s in response to the given question $q$, i.e. $p_K(k | q; \theta)$.}
However, the challenge is that we have no gold knowledge labels as supervision.

\input{floats/ppo}
% \input{floats/ppoo}

\paragraph{Training.}
% \hanna{In training explain that groundtruth labels for k is not available. Instead, you rely on gpt3 output that provides weakly annotated labels for k. Still, this has limitations because first it is not groundtruth, also you need domain-specific prompts to collect these annotations. Therefore, you use RL to supervise knowledge generation as a reward fuction that relies on the  groundtruth labels for answers.}
Since we do not have gold knowledge to train \methodname{}, we obtain this model by finetuning a pretrained language model in two stages: (I) imitation learning, and then (II) reinforcement learning.
In Stage I (\S\ref{sec:method_imit}), we get \dif{\textit{silver}}
% \yejin{weak -> silver? (and also fix the later mentions of `weak'}
knowledge labels on some datasets from GPT-3, and teach our model to imitate this knowledge-generating GPT-3.
This equips our model with the basic functionality of knowledge generation.
In Stage II (\S\ref{sec:method_rl}),
% \hanna{we use reinforcement learning to continue training the model obtained in Stage I, where the reward function is the impact of ... ...}
% we continue training the model obtained in Stage I by optimizing the impact of the
% \dif{we use reinforcement learning to continue training the model, where the reward is the effect of model's}
% generated knowledge on the prediction made by a fixed, generic QA model, so that the knowledge become more useful while staying fluent and meaningful.
% \ximing{this above sentence is a bit long and a bit confusing, trying to break it down...}
we use reinforcement learning to continue training the model obtained in Stage I to make the generated knowledge more useful while staying fluent and meaningful. Specially, we set the reward to be the effect of the generated knowledge on the prediction made by a fixed, generic QA model.
We obtain silver knowledge and train \methodname{} on the union of multiple QA datasets (which are considered \textit{seen} during training), i.e. $\Ds_{\text{seen}} = \bigcup_{d=1}^{\Delta_{\text{seen}}}{\Ds_{d}}$, where $\Ds_d = \{ (q_j, A_j, a^*_j) \}_{j=1}^{|\Ds_d|}$.
%i.e. $\Ds_{\text{ID}} = \bigcup_{d=1}^{\Delta_{\text{ID}}}{\Ds_{d}}$, where $\Ds_d = \{ x_j : x_j = (q_j, A_j, a^*_j) \}_{j=1}^{|\Ds_d|}$.
% \ximing{maybe "\textit{in-domain} QA datasets" is clear enough, probably we don't need the complex notation?}\ximing{We obtain silver knowledge and train \methodname{} on the union of some \textit{in-domain} QA datasets, refered as $\Ds_{\text{ID}}$}
The generic QA model we use may or may not have been trained on these seen datasets.
The complete training process is outlined in Algorithm~\ref{alg:ppo}.

\paragraph{Inference.}
% \hanna{explain that inference you can evaluate on out of domain where no gpt3 labels are available, etc.}
The effectiveness of \methodname{} is evaluated against a set of \textit{unseen} QA datasets, $\Ds_{\text{unseen}}$, in addition to the seen datasets.
Note that \methodname{} is not trained on any unseen datasets, which means we neither get silver knowledge, nor do imitation learning or reinforcement learning on them.
The generic QA model we use was not trained on any unseen datasets as well.
We discuss details of inference in \S\ref{sec:method_inf}.

% \hanna{Start a new paragraph here, say knowledge generator; we also need a bit overview of what is it that the stage 1 trying to imitate, and step 2, what is it that it is reinforcing. something like imitation learning from knowledge statements generated by GPT3 in in-domain data; also you need to bring up the intuition why we have these two steps; you probably can argue we don't have annotated knowledge therefore we rely on GPT3 generated knowledge for imitation learning and then use reinforcement learning to improve. }

\subsection{Training Stage I: Imitation Learning}
\label{sec:method_imit}

In Stage I, we train \methodname{} so that it generates fluent and meaningful natural language statements that resemble knowledge.
\dif{There is no large-scale commonsense QA dataset labeled with high-quality knowledge, but GPT-3 has been shown as a good generator for relevant knowledge \citep{liu2021generated}.}
Therefore, we get silver knowledge from GPT-3 on our seen datasets. % , and train our model to imitate GPT-3's behavior.
% \yejin{we need to better justify why GPT-3: because prior research reported that it's the best knowledge source for commonsense QA benchmarks, to the point of being able to enhance performance even over SOTA models} 
Following \citet{liu2021generated}, we elicit question-related knowledge by prompting GPT-3 with a task-specific set of few-shot demonstrations (See \S\ref{sec:prompts} for details on the prompts), and decoding $M$ knowledge for each question:
% In the first stage, we teach the knowledge generator to imitate the behavior of GPT-3 that is prompted for knowledge generation purpose.
% \citet{liu2021generated} proposed to generate question-relevant knowledge statements by prompting GPT-3 with a task-specific set of few-shot demonstrations.
% Following this approach, we materialize the behavior of GPT-3 by generating a set of knowledge statements for each question in our in-domain datasets:
\begin{align*}
K(q) &= \big\{ k_m : k_m \sim p_G(k \mid \text{prompt}(\text{task}(q)), q) \big\}, % \\ & \qquad \qquad m = 1 \hdots M \big\},
\end{align*}
% \yejin{we could omit m = 1,...M especially that we won't even define what M is and that this detail doesn't seem important} \gary{Added a mention of M above}
where $p_G(\cdot | \cdot)$ denotes GPT-3 with nucleus sampling where $p = 0.5$ \citep{holtzman2019curious}.
This yields a silver dataset of question-knowledge pairs:
%\begin{align}
%\Ds_{\text{imit}}^{s} &= \Big\{ (q, k) : (q, A, a^*) \in \Ds_{\text{ID}}^s, k %\in K(q) \Big\},
%\label{eqn:Dimit-construction}
%\end{align}
\begin{align}
\Ds_{\text{imit}} &= \Big\{ (q, k) : (q, A, a^*) \in \Ds_{\text{seen}}, k \in K(q) \Big\},
\label{eqn:Dimit-construction}
\end{align}
%where $s \in \{ \text{train}, \text{dev} \}$ is the dataset split. 
%\ximing{can we move the split info to appendix and similify the notation?}

We then train \methodname{}, starting from a pretrained sequence-to-sequence language model, on this silver dataset with standard supervised loss: 
%\ximing{maybe we can mention we used T5?}
%\begin{align}
% \mathcal{L}^{\text{train}}(\theta) &= \frac{1}{|\Ds_{\text{imit}}^{\text{train}}|} \sum_{(q, k) \in \Ds_{\text{imit}}^{\text{train}}}{\frac{-\log{p_K(k | q; \theta)}}{|k|}}.
%\mathcal{L}^{\text{train}}(\theta) &\propto \sum_{(q, k) \in %\Ds_{\text{imit}}^{\text{train}}}{\frac{-\log{p_K(k | q; \theta)}}{|k|}}.
%\label{eqn:imit-loss}
%\end{align}
% \vspace{-1mm}
\begin{align}
\mathcal{L}^{\text{train}}(\theta) &\propto \sum_{(q, k) \in \Ds_{\text{imit}}^{\text{train}}}{-\log{p_K(k | q; \theta)}}.
\label{eqn:imit-loss}
\end{align}
% \vspace*{-1mm}
% \yejin{a cleaner way to write this equation is to drop the normalization and just use $\propto$}
%Finally, the model checkpoint with the minimal validation loss, $\mathcal{L}^{\text{dev}}(\theta)$, is selected to initialize Stage II training. %\ximing{maybe we omit checkpoint selection in main text and move to appendix}
%We denote its parameterization as $\theta_{\text{imit}}$.
The parameterization of the resulting model is denoted as $\theta_{\text{imit}}$.

\subsection{Training Stage II: Reinforcement Learning}
\label{sec:method_rl}

% \citet{liu2021generated} showed that knowledge statements generated by few-shot GPT-3 are good prompts for boosting the performance of QA models.
% However,
As we will see in the empirical results, the imitation model obtained in Stage I does not provide the most beneficial knowledge.
Therefore, in Stage II, we continue optimizing \methodname{} to generate  knowledge that \textit{best} prompts the QA model, by directly maximizing the reward given by this QA model.
%as indicated by the reward given by this QA model.
% \hanna{also hint at the point that you use the answer model as a reward here.}
% Suppose we have a fixed QA model that already has reasonable capability to handle the in-domain tasks (i.e. can assign a probability score $\Pqa{a | q}$ to any candidate answer $a \in A$).
% Our goal is to maximize $\Pqa{a^* | q \circ k}$, the probability score received by the correct answer when the QA model is \textit{prompted} with the knowledge, for $k \sim p_K(k | q; \theta)$, where $\circ$ is the text concatenation function specific to the QA model.

\paragraph{Knowledge generation as reinforcement learning.}
Since knowledge statements ($k$'s) are discrete and thus non-differentiable, we adopt a reinforcement learning approach, and consider knowledge generation as a sequential decision making process over the natural language vocabulary space.
We consider the generation of knowledge statement $k$ with  $T$ tokens as an episode of length $T$.
%An episode of length $T$ would be the generation of knowledge statement $k$ with $|k| = T$ tokens.
At step $t \in [1, T]$, the state $s_t = (q, k_{<t})$ is the combination of the question and the knowledge decoded up to the $(t-1)$-th token; the action $a_t = k_t$ would be the $t$-th token to decode.
The \methodname{} model, $p_K(k_t | q, k_{<t}; \theta)$, \dif{is}
% \yejin{would be -> is}
the \textit{policy model} that we optimize.
%We assume there is a reward function
We define a reward function $r(x, k)$ that characterizes the effect of the knowledge on the QA model's prediction, and discuss the definition of this reward function in \S\ref{sec:reward}.
% We define the reward function as the gain of score as received by the correct answer:
% \begin{align}
% r(x, k)
% &= p_{\text{QA}}(a^* | [q || k]) - p_{\text{QA}}(a^* | q) \\
% p_{\text{QA}}(a^* | \cdot)
% &= \frac{l_{\text{QA}}(a^* | \cdot)}{\sum_{a \in A_q}{l_{\text{QA}}(a | \cdot)}}
% \end{align}

% \hanna{in the last paragraph or a new paragraph, you argue you want to cast this problem as a RL setting; then explain what are actions/states, etc. you just mention reward; also tell us what is that you are trying to learn and define the policy.}

% \hanna{what is initial policy; you mean the generated text; explain the intuition why you don't want it to be far from the initial policy}
To ensure that the generated knowledge stay fluent and meaningful, we would like the learned policy model not to move too far from the initial imitation model.
Therefore, we add to the reward an (approximate) KL penalty between the learned policy and the initial policy \citep{ouyang2022training},
%Therefore, we add an entropy bonus term to the reward \citep{ouyang2022training},
\begin{align*}
R(x, k) = r(x, k) - \beta \log{\frac{p_K(k | q; \theta)}{p_K(k | q; \theta_{\text{imit}})}}.
\end{align*}
% where $\theta_{\text{imit}}$ parameterizes the imitation model obtained in Stage I.
Since this reward is computed based on the full knowledge statement, we assign it to the last step of the episode.
Non-terminal steps are assigned zero rewards.
Formally,
\begin{align*}
r_T &= R(x, k) & (\text{where } T = |k| \text{ and } k_T = \text{[EOS]}); \\
r_t &= 0 & (\text{where } 1 \le t < T).
\end{align*}

% \hanna{add a paragraph title Proximal Policy Optimization}
% \paragraph{Proximal Policy Optimization.} \hanna{add a line here or in the footnote why you chose PPO among other RL methods; I can think of statements like we employ PPO as it has shown successful restuls in other NLP tasks; or our earlier investigations with Reinforce didn't show successful results.}

We employ Proximal Policy Optimization\footnote{\dif{We choose PPO because it has shown successful results in other NLP tasks \citep{nakano2021webgpt, stiennon2020learning}. Our earlier experiments with REINFORCE did not show promising results.}} (PPO) \citep{schulman2017proximal} as our reinforcement learning algorithm, and adapt from the implementation of PPO in \citet{ouyang2022training}.
% \hanna{From here on, it is kind of messy with too many equations which are not clear what equations are specific to your model, what is part of the original PPO; you need to organize things;  it is better to first mention what you are optimizing as your PPO loss, and then explain what is your Lpolicy and what is your Lvalue, and why you need the Lvalue; also remember many NLP folks might not know what is value function vs. policy etc. you want to explain them in a paragraph before that casting knowledge generation as RL.}
Aside from the policy model, PPO additionally uses a \textit{value model} (parameterized by $\phi$) to estimate the value function for states with incomplete decoded text, i.e. $V(s_t; \phi)$ for any $t$.
PPO minimizes a joint loss,
\begin{align}
\mathcal{L}_{\text{PPO}}(\theta, \phi) &= \mathcal{L}_{\text{Policy}}(\theta) + \alpha \cdot \mathcal{L}_{\text{Value}}(\phi),
\label{eqn:ppo-loss}
\end{align}
where $\mathcal{L}_{\text{Policy}}(\theta)$ is the loss on the policy model, $\mathcal{L}_{\text{Value}}(\phi)$ is the loss on the value model, and $\alpha$ is a hyperparameter.

\paragraph{Policy loss.}
% To obtain the policy loss, we first follow PPO's definition of the \textit{estimated advantage function}, % \hanna{Q is not defined; instead write this equation as the first line, and then say where Q = \sum....}
% \begin{align*}
% \hat{A}_t
% &= -V(s_t; \phi) + Q(s_t, k_t),
% \end{align*}
% where $Q$ is the action-value function,
% \begin{align*}
% Q(s_t, k_t) &= \sum_{t'=t}^{T-1}{\gamma^{t'-t} r_{t'}} + \gamma^{T-t} V(s_T; \phi).
% \end{align*}
% In the equations above, the the value functions are estimated by the value model.
% In practice, PPO uses the truncated version of the advantage function estimator, 
% \begin{align*}
% & \hat{A}_t = \sum_{t'=t}^{T-1}{(\gamma \lambda)^{t'-t} \delta_{t'}} \\
% % \delta_t + (\gamma \lambda) \delta_{t+1} + \hdots + (\gamma \lambda)^{T-t+1} \delta_{T-1} \\
% & \text{where} \quad \delta_{t'} = r_{t'} + \gamma V(s_{t'+1}; \phi) - V(s_{t'}; \phi).
% \end{align*}
\dif{
%To obtain the policy loss, we first follow PPO's definition of the \textit{truncated estimated advantage function},
To obtain the policy loss, we first compute the \textit{truncated estimated advantage function},
% \vspace*{-2mm}
\begin{align*}
& \hat{A}_t = \sum_{t'=t}^{T-1}{(\gamma \lambda)^{t'-t} \delta_{t'}}, \\
& \text{where} \quad \delta_{t'} = r_{t'} + \gamma V(s_{t'+1}; \phi) - V(s_{t'}; \phi),
\end{align*}
where the value functions \dif{$V(\cdot)$} are estimated by the value model.
}
% \yejin{did you mean to say advantage functions are estimated by the value model? if the answer is no, please add variable names next to the mention of value functions and value models to clarify which is which}
PPO then maximizes the empirical expectation of a so-called \textit{clipped surrogate objective} term,
\begin{align*}
&\text{cso}(\hat{A}_t, \nu_t(\theta), \eps) = \\ &\qquad \min \big( \nu_t(\theta) \hat{A}_t, \text{clip}(\nu_t(\theta), 1 - \eps, 1 + \eps) \hat{A}_t \big),
\end{align*}
where $\nu_t(\theta) = \frac{p_K(k_t | q; \theta)}{p_K(k_t | q; \theta_{\text{old}})}$ is the ratio between the current policy $\theta$ and a lagging policy $\theta_{\text{old}}$.
The lagging policy is updated to the current policy under a fixed interval of $s$ training steps, and is kept fixed otherwise.
% \yejin{we can remove the parenthesis (they should be used extremely sparingly}
We adapt this to our use case, and define the policy loss as
% Formally, we optimize the empirical expectation of a \textit{clipped surrogate objective},
\begin{align*}
% \mathcal{L}_{\text{Policy}}(\theta) &= -\hat{\E} \Big[ \min \big( \nu_t(\theta) \hat{A}_t, \\ & \qquad \qquad \text{clip}(\nu_t(\theta), 1 - \eps, 1 + \eps) \hat{A}_t \big) \Big],
\mathcal{L}_{\text{Policy}}(\theta) &= -\hat{\E} \Big[ \text{cso}(\hat{A}_t, \nu_t(\theta), \eps) \Big]
\end{align*}
where the expectation is taken over all instances in the training data ($x \sim \Ds_{\text{seen}}^{\text{train}}$), the distribution of model-generated knowledge as determined by the current policy conditioning on the instance's question ($k \sim p_K(k | q; \theta)$), and all tokens in the knowledge statement ($t \in [1, |k|]$).
% where $\nu_t(\theta) = \frac{p_K(k_t | q; \theta)}{p_K(k_t | q; \theta_{\text{old}})}$ is the ratio between the current policy $\theta$ and a lagging policy $\theta_{\text{old}}$, and $\hat{A}_t$ is the estimated advantage function at step $t$,
% \begin{align}
% \hat{A}_t
% &= -V(s_t) + Q(s_t, k_t) \\
% &= -V(s_t) + r_t + \gamma r_{t+1} + \hdots + \gamma^{T-t+1} r_{T-1} + \gamma^{T-t} V(s_T)
% \end{align}
% where $s_t = (q, k_{\le t})$.
% In practice, we use the truncated version of the advantage function estimator \citep{schulman2017proximal},
% \begin{align}
% & \hat{A}_t = \delta_t + (\gamma \lambda) \delta_{t+1} + \hdots + (\gamma \lambda)^{T-t+1} \delta_{T-1} \\
% & \text{where} \quad \delta_t = r_t + \gamma V(s_{t+1}) - V(s_t)
% \end{align}

\paragraph{Value loss.}
% Since the value function for incomplete knowledge statements is indeterminable, we use a separate \textit{value model} $V(s_t; \phi)$ to estimate the value function.
The value model is trained with MSE loss with respect to the target value, $V^{\text{targ}}_t$, which in turn is estimated with a lagging value model $\phi_{\text{old}}$:
\begin{align*}
& \mathcal{L}_{\text{Value}}(\phi) = \hat{\E} \Big[ \big( V(s_t; \phi) - V^{\text{targ}}_t \big)^2 \Big], \\
& \text{where} \quad V^{\text{targ}}_t = \sum_{t'=t}^{T-1}{\gamma^{t'-t} r_{t'}} + \gamma^{T-t} V(s_T; \phi_{\text{old}}).
\end{align*}
% where $\phi_{\text{old}}$ parameterizes a lagging value model.

% Finally, the knowledge generation policy model and the value model are jointly trained to minimize the PPO loss,
% \begin{align}
% \mathcal{L}_{\text{PPO}}(\theta, \phi) &= \mathcal{L}_{\text{Policy}}(\theta) + \alpha \cdot \mathcal{L}_{\text{Value}}(\phi)
% \end{align}

\subsubsection{Reward Shaping}
\label{sec:reward}

\dif{
We define the reward function in reinforcement learning as the quantified effect of \methodname{}'s knowledge on the QA model's prediction.
Suppose we already have a reasonably good QA model, which assigns a probability score $\Pqa{a|q}$ to any candidate answer $a \in A$.
% As mentioned in \S\ref{sec:method_rl}, we need a QA model that can assign a probability score $\Pqa{a|q}$ to any candidate answer $a \in A$.
Since we will use a sequence-to-sequence language model (i.e. UnifiedQA \citep{khashabi2020unifiedqa}) as the QA model, we define
\begin{align*}
\Pqa{a | q} = \frac{\exp{\Sqa{a | q}}}{\sum_{a' \in A}{\exp{\Sqa{a' | q}}}},
\end{align*}
where
\begin{align*}
\Sqa{a | q} = \frac{1}{|a|} \sum_{i=1}^{|a|}{-\log{\pqa{a_i | q, a_{<i}; \psi_{\text{QA}}}}},
\end{align*}
where $\pqa{a_i | q, a_{<i}; \psi_{\text{QA}}}$ is the language modeling score received by $a_i$, the $i$-th token of $a$.
The naive prediction would be the candidate answer that gets the highest $\Pqa{a|q}$ (or equivalently, the highest $\Sqa{a|q}$): $\hat{a} = \argmax_{a \in A} \Pqa{a | q}$.
}

\dif{
We aim at maximizing $\Pqa{a^* | q \circ k}$, the probability score received by the correct answer when the QA model is prompted with the knowledge $k$ generated by \methodname{}, and $\circ$ denotes text concatenation.
One naive definition of reward function may be
\begin{align*}
r(x, k) = \Pqa{a^* | q \circ k} - \Pqa{a^* | q}.
\end{align*}
However, this reward only captures the absolute change of score, but not whether the model prediction is changed or not.
To remedy for this, we define the reward function as
\begin{align*}
& r(x, k) = \frac{1}{2} \Big[ \\
& \quad \tanh \big( \Sqa{a^* | q \circ k} - \max_{\substack{a' \in A, \\ a' \ne a^*}} \Sqa{a' | q \circ k} \big) \\ & \quad - \tanh \big( \Sqa{a^* | q} - \max_{\substack{a' \in A, \\ a' \ne a^*}} \Sqa{a' | q} \big) \Big].
\end{align*}
Intuitively, this function would give a reward of near $+1$ if the naive prediction is incorrect (i.e. $\Sqa{a^* | q} < \max_{a' \in A, a' \ne a^*} \Sqa{a' | q}$), while the knowledge-prompted prediction is correct (i.e. $\Sqa{a^* | q \circ k} > \max_{a' \in A, a' \ne a^*} \Sqa{a' | q \circ k}$).
Similarly, the reward would be near $-1$ if the naive prediction is correct but the knowledge-prompted prediction is incorrect.
The hyperbolic tangent serves as a smoothed sign function, and provides a soft interpolation between the two polarity of reward values by taking into account the margin of the correct answer.
}

We also experiment with some alternative definitions of the reward function. See \autoref{tab:ablation_rewards}.
% \begin{align*}
% \text{Prob only: } & r(x, k) = \Pqa{a^* | q \circ k} \\
% \text{Prob diff: } & r(x, k) = \Pqa{a^* | q \circ k} - \Pqa{a^* | q} \\
% \text{Score diff: } & r(x, k) = \Sqa{a^* | q \circ k} - \Sqa{a^* | q} \\
% \text{Uniform reference: } & r(x, k) = \frac{1}{2} \Big[ \tanh \big( \Pqa{a^* | q \circ k} - \frac{1}{|A|} \big) - \tanh \big( \Pqa{a^* | q} - \frac{1}{|A|} \big) \Big] \\
% \text{Hard activation: } & r(x, k) = \frac{1}{2} \Big[ \sgn \big( \Sqa{a^* | q \circ k} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q \circ k} \big) \\ & \qquad - \sgn \big( \Sqa{a^* | q} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q} \big) \Big]
% \end{align*}

% We propose the following candidate formulations of the reward function:
% \begin{align*}
% 0: r(x, k) &= \Pqa{a^* | q \circ k} - \Pqa{a^* | q} \\
% 1: r(x, k) &= \Pqa{a^* | q \circ k} \\
% 2: r(x, k) &= \Sqa{a^* | q \circ k} - \Sqa{a^* | q} \\
% 3: r(x, k) &= \Sqa{a^* | q \circ k} \\
% 4: r(x, k) &= \frac{1}{2} \Big[ \tanh \big( \Sqa{a^* | q \circ k} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q \circ k} \big) \\ & \qquad - \tanh \big( \Sqa{a^* | q} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q} \big) \Big] \\
% 5: r(x, k) &= \frac{1}{2} \Big[ \sgn \big( \Sqa{a^* | q \circ k} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q \circ k} \big) \\ & \qquad - \sgn \big( \Sqa{a^* | q} - \max_{a' \in A, a' \ne a^*} \Sqa{a' | q} \big) \Big] \\
% 6: r(x, k) &= \frac{1}{2} \Big[ \tanh \big( \Pqa{a^* | q \circ k} - \frac{1}{|A|} \big) - \tanh \big( \Pqa{a^* | q} - \frac{1}{|A|} \big) \Big] \\
% 7: r(x, k) &= \frac{1}{2} \Big[ \sgn \big( \Pqa{a^* | q \circ k} - \frac{1}{|A|} \big) - \sgn \big( \Pqa{a^* | q} - \frac{1}{|A|} \big) \Big] \\
% 8: r(x, k) &= \frac{1}{|a^*|} \sum_{i=1}^{|a^*|}{\frac{1}{2} \Big[ \tanh \big( \sqa{a^*_i | q \circ k, a^*_{<i}} - \max_{a'_i \in V, a'_i \ne a^*_i} \sqa{a'_i | q \circ k, a^*_{<i}} \big)} \\ & \qquad \qquad \qquad - \tanh \big( \sqa{a^*_i | q, a^*_{<i}} - \max_{a'_i \in V, a'_i \ne a^*_i} \sqa{a'_i | q, a^*_{<i}} \big) \Big] \\
% 9: r(x, k) &= \frac{1}{|a^*|} \sum_{i=1}^{|a^*|}{\frac{1}{2} \Big[ \sgn \big( \sqa{a^*_i | q \circ k, a^*_{<i}} - \max_{a'_i \in V, a'_i \ne a^*_i} \sqa{a'_i | q \circ k, a^*_{<i}} \big)} \\ & \qquad \qquad \qquad - \sgn \big( \sqa{a^*_i | q, a^*_{<i}} - \max_{a'_i \in V, a'_i \ne a^*_i} \sqa{a'_i | q, a^*_{<i}} \big) \Big]
% \end{align*}

\paragraph{Reward normalization.}
To stabilize training, we apply an affine transformation on the rewards so that initially they are normalized.
Before starting Stage II training, we use the imitation model to generate a knowledge statement for each training instance, and estimate the population mean and standard deviation of rewards:
\begin{align}
\mathcal{R}_{\text{init}} &= \big\{ r(x, k) : x \in \Ds_{\text{seen}}^{\text{train}}, k \sim p_K(\cdot | q; \theta_{\text{imit}}) \big\}, \nonumber \\
\mu_0 &= \mu(\mathcal{R}_{\text{init}}), \sigma_0 = \sigma(\mathcal{R}_{\text{init}}).
\label{eqn:reward-norm-compute}
\end{align}
In Stage II training, each reward is normalized as:
\begin{align}
r(x, k) &\leftarrow \frac{r(x, k) - \mu_0}{\sigma_0}.
\label{eqn:reward-norm-apply}
\end{align}

\subsection{Inference: Knowledge Prompting and Aggregation}
\label{sec:method_inf}

Following \citet{liu2021generated}, at inference time we use \methodname{} to generate multiple knowledge per question, and \textit{prompt} the QA model by individually concatenating each knowledge to the question.
The knowledge are generated by \methodname{} with nucleus sampling where $p = 0.5$ \citep{holtzman2019curious},
\begin{align*}
K(q) &= \{\eps\} \cup \big\{ k_m : k_m \sim p_K^{p=0.5}(k \mid q; \theta), \\
& \qquad \qquad \qquad \quad m = 1 \hdots M \big\},
\end{align*}
% \yejin{could remove m=1,,,M for brevity}
where $M$ is the number of knowledge per question, and $\eps$ denotes empty string.
We collect a set of outputs for prompting with each knowledge.
The final prediction is the candidate answer that receives maximum confidence,
\begin{align*}
\hat{a} &= \argmax_{a \in A} \max_{k \in K(q)} \Pqa{a | q \circ k},
\end{align*}
and the prediction is supported by a single knowledge -- the \textit{selected knowledge},
% \vspace{-0.5mm}
\begin{align*}
\hat{k} &= \argmax_{k \in K(q)} \max_{a \in A} \Pqa{a | q \circ k}.
\end{align*}

\paragraph{Training time model selection.}
In Stage II training, we only generate one knowledge per question for the validation set.\footnote{This is for efficiency purposes. We use greedy decoding here because it is more stable than nucleus sampling when generating only one knowledge per question.}
% , using greedy decoding. \yejin{why greedy here? (whereas nucleus used just a paragraph ago?)} \gary{Emm, this is what we did. If we're only generating 1 knowledge, then greedy is more stable than nucleus. But if this complicates things, maybe we can just omit this mention?}
Predictions are made using the same knowledge prompting method as above, and the model checkpoint with the maximal accuracy on the union of all validation sets is selected.

==> [EMNLP 2022] cc-GKM/sections/related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Explicit reasoning for commonsense QA.}
Commonsense question answering poses a significant challenge to modern neural models.
To improve performance and interpretability, many work have proposed to do explicit reasoning for tasks in this area, that is, to verbalize the intermediate text artifacts that facilitate the reasoning process.
\citet{rajani2019explain} and \citet{latcinnik2020explaining} use supervised learning to train models to generate text explanations, while \citet{gu2021dream} and \citet{bansal2021cose} use similar training regimes to obtain models that can generate scene elaborations and paths through a structured knowledge graph, respectively.
\citet{shwartz2020unsupervised} and \citet{paranjape2021prompting} prompt pretrained models with pre-defined templates to generate question clarifications or contrastive explanations, which are in turn used to prompt the inference model.
The above approaches all \dif{pose, implicitly or explicitly, certain constraints (e.g. domain, relation, syntax) on the model-generated text.}
% assume, implicitly or explicitly, an \textit{a priori} nature of the model-generated text.\
% \yejin{the meaning of `a priori nature of model-generated text' isn't clear to me... (I think I can guess what it means, but somehow that doesn't click with the above paragraph for me, and I suspect that many readers might have similar confusion)}
In contrast, \citet{wei2022chain} elicits full chain-of-reasoning from language models with in-context learning; \citet{liu2021generated} uses few-shot demonstrations to elicit flexible, relevant knowledge statements from a language model, and \citet{wang2022elaboration} distills this capability into smaller models using supervised learning.
These methods provide more flexibility on the knowledge, yet they rely on accessing very large language models (e.g. GPT-3).
Aside from methods that make reasoning explicit in a linear chain manner, another set of work produce recursive structures of reasoning, through either backward chaining \citep{dalvi2022towards, jung2022maieutic} or forward chaining \citep{bostrom2022natural}.
\dif{Our work contributes to this line of research, yet we depart from prior work by presenting the first approach that \textit{learns} to generate relevant knowledge without requiring human-labeled gold knowledge.}
% Our work follows from this line of research, and focuses on building a unified model that can flexibly generate arbitrary types of relevant knowledge for commonsense questions across a variety of domains.
% \yejin{the last sentence isn't precise enough, as it sounds as if we unify all the previous approaches, even including e.g., chain of thoughts. can we instead better highlight that ``we depart from the prior work by demonstrating the first approach that *learns* to generate relevant knowledge without requiring human-annotated gold knowledge''}

\paragraph{Reinforcement learning for NLP.}
Recently, reinforcement learning methods have been adopted for NLP tasks like question answering \citep{nakano2021webgpt}, summarization \citep{stiennon2020learning, paulus2017deep}, machine translation \citep{shen2015minimum, wu2016google}, grounded text generation \citep{ammanabrolu2020motivate, ammanabrolu2022aligning}, controlled text generation \citep{lu2022quark}, and prompt generation \citep{guo2021text, deng2022rlprompt}.
% To our knowledge, we are the first to train models with reinforcement learning to dynamically generate free-form knowledge.
% \yejin{the enumeration of RL applications for almost random NLP applications is a tad too basic and almost uninteresting... can we instead say something more concretely about PPO for NLP applications, and go a bit deeper into how ours stand out compared to recent prior work?}
Our application of reinforcement learning on knowledge introspection is novel.
The idea of reinforcement learning with model-provided feedback has been previously explored in \citet{guo2021text}, \citet{ammanabrolu2020motivate}, and \citet{lu2022quark}.
The PPO algorithm has been previously employed to optimize rewards learned from human feedback \citep{nakano2021webgpt, stiennon2020learning}.
In contrast, we use PPO to optimize reward purely derived from the decision-making neural models.

% \paragraph{Free text knowledge bases.}


==> [EMNLP 2022] cc-GKM/sections/results.tex <==
\section{Results}
\label{sec:results}

\subsection{Main Results}
\label{sec:result_main}

% \hanna{1. the setup is not clear; zero-shot vs. fine-tuned; all these need to be better explained in the setting and also in the overview paragraph in the method section. 2. why we are only comparing with GPT3-knowledge in some cases not all of them?}

\input{floats/results}
\paragraph{Performance on seen datasets.}
\autoref{tab:results_id} shows the performance of \methodname{}-enhanced QA model on the seen datasets.
On average, our method achieves more than 5\% improvement over directly applying the QA model.
The knowledge generated by \methodname{} improves performance on five benchmarks: CommonsenseQA, QASC, PhysicalIQA, SocialIQA, and Winogrande, with the greatest improvement on CommonsenseQA (+6\%) and QASC (+12\%).
As shown in \autoref{tab:results_id_nope}, there is no performance gain on OpenBookQA, ARC, and AI2Science.
We conjecture that this is because the QA model, UnifiedQA, is already trained on these three datasets, thus setting a strong baseline.

\paragraph{Comparison with other models.}
Compared to \methodname{}, other knowledge generation models, including few-shot GPT-3, Self-talk, and DREAM, provide generally weaker improvements over the vanilla QA baseline.
In particular, \methodname{} outperforms GPT-3-based models
% The few-shot GPT-3 knowledge generator is only able to provide small improvement on CommonsenseQA, QASC, and Winogrande, while hurting the performance on other benchmarks.
% This has been shown in \citet{liu2021generated}, as the 13B version of GPT-3 serves as a weaker knowledge generator.
% In contrast, \methodname{} can provide larger and more consistent improvements, 
while being 16x smaller in parameter size (0.77B vs. 13B).

\paragraph{Performance on unseen datasets.}
\autoref{tab:results_ood} shows that \methodname{}'s knowledge substantially improves performance over the vanilla QA baseline on the four unseen datasets, demonstrating its generalization capability.

\input{floats/results_qa}
\paragraph{Choice of QA model for evaluation.}
To verify that our \methodname{} model is not hacking into the rewards provided by the QA model we use during training, we evaluate the effect of \methodname{}'s knowledge on different QA models.
We choose three other UnifiedQA models with different sizes, as well as a different model known as Unicorn \citep{lourie2021unicorn}.
Results are shown in \autoref{fig:results_qa}.
\methodname{} consistently gives performance gains on top of all QA models, indicating that its knowledge are generally useful information rather than mere artifacts of model-specific reward hacking.
% \hanna{it is a bit too strong; still you are only using different sizes of uqa, but not other qa models. maybe they have some shared behavior. tone down this last sentence.}
We even observe performance gains with a QA model that is 4x as large as \methodname{}, which means generating and prompting relevant knowledge can be a technique complementary to model scaling, and can be done meaningfully with smaller models.
Finally, we see the largest improvement when the QA model itself has weak, but non-trivial, performance (UnifiedQA-small for seen datasets, and UnifiedQA-base for unseen datasets).

\subsection{Ablations}
\label{sec:ablations}

% \paragraph{Choice of QA model for training.}

\input{floats/ablations}

\paragraph{Stage I and Stage II training.}
We experimented with omitting the Stage I (imitation) and/or Stage II (reinforcement) from the training pipeline.
Results are shown in \autoref{tab:ablation_stages}.
Without Stage I training, \methodname{} does not improve the performance of the QA model \dif{(regardless of whether it is trained with Stage II or not)}, showing the indispensability of equipping the model with the basic functionality of knowledge generation.
On the other hand, a model trained solely with Stage I gives weaker improvements than the fully trained \methodname{}, stressing the importance of Stage II training as well.
% \hanna{what is -stage1-stage2? is it going to be simialr to uqa alone? }

\paragraph{Reward function.}
\autoref{tab:ablation_rewards} shows the results for knowledge introspectors trained with different reward functions.
Our reward shaping gives the best performance on unseen datasets, as well as one of the top performance on seen datasets.
% \hanna{maybe you want to mention something for the prob. diff that gives the higher in domain, and mentioning that your reward shaping help to generazlie better to ood}
\dif{While the naive \textit{prob diff} reward function gives slightly better performance on seen datasets, our reward shaping results in better generalization.}

\subsection{Analysis}
\label{sec:analysis}

\input{floats/human}
% \input{floats/human_cats}

\dif{
To get a deeper understanding of the behavior and capability of \methodname{}, we manually analyzed the generated knowledge along several \textbf{quality} and \textbf{diversity} aspects.
% \hanna{move this paragraph at the beginning of where you explain the rectify/mislead results and call it a new paragraph... Impact of generated knowledge or someting?}
% We annotated the \textit{selected knowledge} (\S\ref{sec:method_inf}) that change the correctness of UnifiedQA-large's prediction (either from wrong to right, a.k.a. \textit{rectifies} model prediction; or from right to wrong, a.k.a. \textit{misleads} model prediction).
% We choose 8 benchmarks (5 in-domain, 3 out-of-domain; see \autoref{fig:human}), and randomly select up to 100 questions whose selected knowledge meet the above criterion.
% Three NLP experts did the annotation, where each knowledge is annotated by one person.
% It was hidden from the annotators whether the knowledge rectifies or misleads the model prediction, so that potential bias is eliminated.
We asked three NLP experts to annotate the \textit{selected knowledge} (\S\ref{sec:method_inf}) for up to 100 questions per dataset among the validation sets of 8 benchmarks (5 seen, 3 unseen; see \autoref{fig:human}).
It was hidden from the annotators whether the knowledge rectifies or misleads QA model's prediction, so potential bias is eliminated.
}

\paragraph{Quality.}
First, we follow \citet{liu2021generated} by annotating the quality aspects -- \textit{relevance}, \textit{factuality}, and \textit{helpfulness} -- of each knowledge with respect to the question.
We find that \methodname{}-generated knowledge are overwhelmingly related to the respective questions.
64\% are factually correct, 25\% are factually incorrect, and the remaining 11\% have undetermined factuality due to various reasons (e.g. ambiguity, cultural sensitivity).
58\% are seen by human as being helpful for reasoning about the question, whereas 24\% are seen as harmful.

% \hanna{not clear to me: what percentage of knowledge rectifies and what percentage of the knowledge misleads?}
\dif{
In our annotations, there are 420 knowledge that \textit{rectify} UnifiedQA-large's predictions (i.e. flipping from wrong to right), and 246 knowledge that \textit{mislead} the predictions (i.e. flipping from right to wrong).
Among the rectifying knowledge, 84\% are deemed helpful by human; and among the misleading knowledge, 62\% are deemed harmful.
These results have similar trends as \citet{liu2021generated}, and show that \methodname{}'s knowledge are of high quality and interpretability in helping QA models.
}
% \hanna{can you compare it with liu et all work? }

\paragraph{Diversity.}
% \hanna{move the paragraph at the beg. of 4.3 that you explain about diversity to here.}
Additionally, we analyze the \textbf{diversity} aspects by annotating each knowledge with the \textit{domain}(s) it belongs to (e.g. scientific, social), the \textit{relation}(s) it expresses (e.g. attribute, capable of), and its \textit{syntactic} property(s) (e.g. negation, comparison).
See \autoref{fig:human} for complete list of options under each aspect.
The knowledge's domain distribution is strongly tied to the domain of the benchmark (e.g. scientific for QASC and QuaRTz, social for SocialIQA and Winogrande, numerical for NumerSense).
The domain aspect is more diverse for benchmarks that test general commonsense, like CommonsenseQA and RiddleSense.
For the relation aspect, there are many knowledge that express an ``attribute'' relation, while other relations are also substantially represented.
As for syntax, a good proportion of the knowledge contain structures like comparison and negation.
Therefore, \methodname{}'s knowledge have good syntactic and semantic diversity while being able to adapt to the domain.

\subsection{Qualitative Examples}
\label{sec:qual}

% \input{floats/qual}

We show some examples of good knowledge generated by \methodname{} in \autoref{tab:qual}.

% \hanna{References are a bit weird; why do we have underlines for the conferences? I didn't notice it in my other submissions.}
% \gary{Ah thanks for bringing this up. Removing the ulem package fixed it.}


==> floats/trash/human_cats.tex <==
\begin{table*}
\centering
\resizebox{0.75 \textwidth}{!}{%
\begin{tabular}{lrrrrrrrrr}
\toprule
& CSQA & QASC & PIQA & SIQA & WG & NS & RS & QuaRTz & \textbf{All} \\
\midrule
\textbf{Domains} \\
scientific & 13\% & 79\% & 6\% & 0\% & 0\% & 20\% & 21\% & 84\% & 25\% \\
social & 24\% & 0\% & 6\% & 94\% & 59\% & 10\% & 9\% & 0\% & 27\% \\
physical & 34\% & 10\% & 11\% & 0\% & 4\% & 0\% & 3\% & 21\% & 12\% \\
temporal & 5\% & 14\% & 0\% & 3\% & 4\% & 0\% & 0\% & 0\% & 4\% \\
numerical & 0\% & 0\% & 3\% & 0\% & 0\% & 90\% & 3\% & 5\% & 5\% \\
\midrule
\textbf{Relations} \\
definition & 5\% & 3\% & 0\% & 0\% & 0\% & 0\% & 35\% & 5\% & 7\% \\
attribute & 39\% & 62\% & 28\% & 39\% & 74\% & 60\% & 32\% & 53\% & 46\% \\
part of & 3\% & 7\% & 3\% & 0\% & 0\% & 30\% & 12\% & 0\% & 5\% \\
member of & 3\% & 7\% & 0\% & 0\% & 0\% & 10\% & 12\% & 0\% & 4\% \\
capable of & 5\% & 7\% & 28\% & 3\% & 0\% & 0\% & 3\% & 5\% & 8\% \\
purpose & 0\% & 7\% & 28\% & 0\% & 0\% & 0\% & 6\% & 5\% & 7\% \\
causality & 3\% & 10\% & 3\% & 0\% & 0\% & 0\% & 0\% & 16\% & 4\% \\
strategy & 11\% & 10\% & 22\% & 3\% & 0\% & 0\% & 0\% & 0\% & 7\% \\
\midrule
\textbf{Syntax} \\
negation & 3\% & 0\% & 6\% & 10\% & 19\% & 10\% & 18\% & 0\% & 8\% \\
comparison & 8\% & 7\% & 17\% & 3\% & 30\% & 0\% & 0\% & 79\% & 16\% \\
condition & 5\% & 0\% & 8\% & 0\% & 0\% & 0\% & 0\% & 11\% & 3\% \\
because & 11\% & 0\% & 3\% & 0\% & 7\% & 0\% & 0\% & 0\% & 3\% \\
\bottomrule
\end{tabular}
}%
\caption{
    Percentage of \methodname{}-generated knowledge categorized by domain, expressed relation, and syntax.
    The percentages do not add up to 100\% because some knowledge have none of these characteristics, while some others may have multiple. \hanna{This table is not readable; first, you don't need all those \%s it just confuses the reader; maybe a bar chart? there are too many numbers here, which makes things harder to read ?or some sort of heatmap?}
    \skyler{I think this would look good as three comparative bar charts: Domain, Relation, and Syntax, so we can see the distribution of each of the datasets}
}
\label{tab:human_cats}
\vspace{-16pt}
\end{table*}

==> floats/trash/hypers_short.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c c p{138pt}}
\toprule
\textbf{Symbol} & \textbf{Value} & \textbf{Description} \\
\midrule
\multicolumn{3}{c}{\textsc{Training Stage I: Imitation Learning}} \\
\midrule
$M$ & 20 & Number of knowledge statements to sample from GPT-3, per question. \\
$p$ & 0.5 & Parameter for nucleus sampling from GPT-3. \\
% $L_{\text{output}}$ & 64 & Max length of output from GPT-3. \\
% $L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
% $L_{\text{output}}$ & 64 & Max length of output from \methodname{} (i.e. generated knowledge). \\
$B$ & 64 & Batch size for training. \\
$S$ & 50,000 & Total number of training steps. \\
$\eta$ & $1 \times 10^{-5}$ & Learning rate of Adam optimizer. \\
\midrule
\multicolumn{3}{c}{\textsc{Training Stage II: Reinforcement Learning}} \\
\midrule
$\alpha$ & 1.0 & Weight of value model loss in PPO. \\
$\beta$ & 0.2 & Weight of entropy bonus term in reward. \\
$\gamma$ & 1.0 & Discount factor for rewards. \\
$\lambda$ & 0.95 & Parameter for advantage estimation. \\
$\eps$ & 0.2 & Clipping range for the \textit{clipped surrogate objective}. \\
% $L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
% $L_{\text{output}}$ & 32 & Max length of output from \methodname{} (i.e. generated knowledge). \\
$\tau$ & 0.7 & Temperature for knowledge sampling in PPO training. \\
% $E$ & 1M & Total number of training episodes. \\
$B$ & 64 & Batch size for training. \\
$S$ & 15,625 & Total number of training steps. \\
% $s$ & 4 & Interval (in steps) for updating the lagging models (policy and value). \\
$\eta$ & $2 \times 10^{-5}$ & Learning rate of Adam optimizer (with a linear learning rate decay schedule). \\
\midrule
\multicolumn{3}{c}{\textsc{Inference}} \\
\midrule
$M$ & 10 & Number of knowledge statements to sample from \methodname{}, per question. \\
$p$ & 0.5 & Parameter for nucleus sampling from \methodname{}. \\
% $L_{\text{input}}$ & 256 & Max length of input to \methodname{} (i.e. question plus choices). \\
% $L_{\text{output}}$ & 32 & Max length of output from \methodname{}. \\
\bottomrule
\end{tabular}
\caption{
    Hyperparameter settings (partial).
    See \autoref{tab:hypers} for full list.
}
\label{tab:hypers_short}
\vspace{-8pt}
\end{table}

==> floats/trash/ppoo.tex <==
\begin{algorithm*}
\small
\caption{Training \methodname{}, Stage II, Reinforcement Learning; \hanna{for this algorithm (you can move it to appendix, but in the main text simplify it a lot; basically you have equations in the text and are repeating it here; Just say Lpolicy calculate through eq. blah blah; LPPo calculate through eq blah blah and remove all the rest of the previous things. you just need to list the big training steps where is the }}
\begin{algorithmic}
\Procedure{ReinforcementLearning}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\phi_0$, $\psi_{\text{QA}}$}
    \Procedure{ComputeRewardNormalizationFactors}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\psi_{\text{QA}}$}
        \State $\mathcal{R}_{\text{init}} \gets \{\}$
        \ForAll {$x = (q, A, a^*) \in \Ds_{\text{ID}}$}
            \State $k \gets$ \Call{TemperatureSampling}{$q$, $\theta_{\text{imit}}$, $\tau$}
            \State $r \gets r(x, k; \psi_{\text{QA}})$
            \State $\mathcal{R}_{\text{init}} \gets \mathcal{R}_{\text{init}} \cup \{ r \}$
        \EndFor
        \State $\mu_0 \gets \mu(\mathcal{R}_{\text{init}})$, $\sigma_0 \gets \sigma(\mathcal{R}_{\text{init}})$
        \State \Return $(\mu_0, \sigma_0)$
    \EndProcedure
    \State $(\mu_0, \sigma_0) \gets$ \Call{ComputeRewardNormalizationFactors}{$\Ds_{\text{ID}}$, $\theta_{\text{imit}}$, $\psi_{\text{QA}}$}
    \State $\theta \gets \theta_{\text{imit}}$, $\phi \gets \phi_0$
    \State $\theta_{\text{old}} \gets \theta$, $\phi_{\text{old}} \gets \phi$
    \For {$i = 1 \hdots S$}
        \State \textit{batch} $\gets$ sample a batch of size $B$ from $\Ds_{\text{ID}}$
        \State $\mathcal{L}_{\text{Policy}} \gets 0$, $\mathcal{L}_{\text{Value}} \gets 0$
        \ForAll {$(q, A, a^*) \in$ \textit{batch}}
            \State $k \gets$ \Call{TemperatureSampling}{$q$, $\theta$, $\tau$}
            \State $r \gets r(x, k; \psi_{\text{QA}})$
            \State $r \gets (r - \mu_0) / \sigma_0$
            \State $R \gets r - \beta \log{\big( p_K(k | q; \theta) / p_K(k | q; \theta_{\text{imit}}) \big)}$
            \State $T \gets |k|$
            \State $r_T \gets R$, $r_{[1 \hdots T-1]} \gets 0$
            \For {$t = T \hdots 1$}
                \State $\delta_t \gets r_t + \gamma V(s_{t+1}; \phi) - V(s_t; \phi)$
                \State $\hat{A}_t \gets \delta_t + (\gamma \lambda) \delta_{t+1} + \hdots + (\gamma \lambda)^{T-t+1} \delta_{T-1}$
                \State $V_t^{\text{targ}} \gets r_t + \gamma r_{t+1} + \hdots + \gamma^{T-t+1} r_{T-1} + \gamma^{T-t} V(s_T; \phi_{\text{old}})$
                \State $\nu_t \gets p_K(k_t | q; \theta) / p_K(k_t | q; \theta_{\text{old}})$
                \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} - \min \big( \nu_t \hat{A}_t, \text{clip}(\nu_t, 1 - \eps, 1 + \eps) \hat{A}_t \big)$
                \State $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} + (V(s_t; \phi) - V_t^{\text{targ}})^2$
            \EndFor
            \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} / T$, $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} / T$
        \EndFor
        \State $\mathcal{L}_{\text{Policy}} \gets \mathcal{L}_{\text{Policy}} / B$, $\mathcal{L}_{\text{Value}} \gets \mathcal{L}_{\text{Value}} / B$
        \State $\mathcal{L}_{\text{PPO}} \gets \mathcal{L}_{\text{Policy}} + \alpha \cdot \mathcal{L}_{\text{Value}}$
        \State $\theta \gets \theta - \eta \cdot \nabla_\theta \mathcal{L}_{\text{PPO}}$, $\phi \gets \phi - \eta \cdot \nabla_\phi \mathcal{L}_{\text{PPO}}$
        \If {$i \equiv 0 (\text{mod } s)$} \Comment{Update the lagging policy every $s$ steps.}
            \State $\theta_{\text{old}} \gets \theta$, $\phi_{\text{old}} \gets \phi$
        \EndIf
        \State \Return $\theta$
    \EndFor
\EndProcedure
\end{algorithmic}
\label{alg:ppoo}
\end{algorithm*}

==> floats/trash/results.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l ccccccccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{OBQA} & \multicolumn{2}{c}{ARC} & \multicolumn{2}{c}{AI2Science} & \multirow{2}{*}{CSQA} & \multirow{2}{*}{QASC} & \multirow{2}{*}{PIQA} & \multirow{2}{*}{SIQA} & \multirow{2}{*}{WG} & \textbf{Avg.} \\
\textbf{Method} $\downarrow$ &  & \small{easy} & \small{hard} & \small{elem} & \small{mid} & & & & & & (last 5) \\
\midrule
UQA & 70.20 & 69.12 & 55.85 & 69.11 & 64.80 & 61.43 & 43.09 & 63.66 & 53.84 & 53.35 & 55.07 \\
\methodname{} (T5-large) + UQA & 69.60 & 67.72 & 55.18 & 68.29 & 63.20 & \textbf{67.24} & \textbf{54.97} & \textbf{65.67} & \textbf{57.01} & \textbf{56.91} & \textbf{60.36} \\
\midrule
Few-shot GPT-3 (13B) + UQA & 68.80 & 71.05 & 56.52 & 70.73 & 65.60 & 66.34 & 53.24 & 64.25 & 58.29 & 55.56 & 59.54 \\
Self-talk GPT-3 (13B) + UQA & -- & -- & -- & -- & -- & 63.31 & 49.89 & 65.23 & 51.89 & 52.96 & 56.66 \\
DREAM (11B) + UQA & -- & -- & -- & -- & -- & 64.54 & 49.46 & 64.74 & 51.59 & 56.12 & 57.29 \\
\bottomrule
\end{tabular}
}%
\vspace{-6pt}
\caption{
    Results on in-domain datasets.
    Accuracy on dev set is reported.
    Predictions made by UQA-large.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_id}
%
\vspace{6pt}
%
\begin{minipage}[t]{.49 \linewidth}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l cccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{CSQA} & \multirow{2}{*}{QASC} & \multirow{2}{*}{PIQA} & \multirow{2}{*}{SIQA} & \multirow{2}{*}{WG} & \multirow{2}{*}{\textbf{Avg.}} \\
\textbf{Method} $\downarrow$ \\
\midrule
UQA & 53.00 & 45.65 & 65.50 & 57.21 & 54.67 & 55.21 \\
\methodname{} (T5-large) + UQA & \textbf{60.18} & \textbf{54.13} & \textbf{67.09} & \textbf{59.01} & \textbf{57.39} & \textbf{60.00} \\
\bottomrule
\end{tabular}
}%
\vspace{-6pt}
\caption{
    Results on in-domain datasets.
    Accuracy on test set is reported.
    Predictions made by UQA-large.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_id_test}
\end{minipage}
%
\hfill
%
\begin{minipage}[t]{.49 \linewidth}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l cccccccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{NS} & \multirow{2}{*}{RS} & \multirow{2}{*}{QuaRTz} & \multirow{2}{*}{HS} & \multirow{2}{*}{\textbf{Avg.}} \\
\textbf{Method} $\downarrow$ \\
\midrule
UQA & 26.50 & 28.11 & 68.75 & 35.00 & 39.59 \\
\methodname{} (T5-large) + UQA & \textbf{30.00} & \textbf{30.07} & \textbf{70.31} & \textbf{35.73} & \textbf{41.53} \\
\midrule
Few-shot GPT-3 (13B) + UQA & 38.00 & 35.65 & 69.01 & 37.33 & 45.00 \\
\bottomrule
\end{tabular}
}%
\vspace{-6pt}
\caption{
    Results on out-of-domain datasets.
    Accuracy on dev set is reported.
    Predictions made by UQA-large.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_ood}
\end{minipage}
%
\vspace{12pt}
%
\centering
\resizebox{0.8 \textwidth}{!}{%
\begin{tabular}{l cccccccccccc}
\toprule
\textbf{QA Model} $\rightarrow$ & \multicolumn{2}{c}{UQA-small} & \multicolumn{2}{c}{UQA-base} & \multicolumn{2}{c}{UQA-large} & \multicolumn{2}{c}{UQA-3b} & \multicolumn{2}{c}{Unicorn-large} \\
\textbf{Knowledge Gen.} $\downarrow$ & ID & OOD & ID & OOD & ID & OOD & ID & OOD & ID & OOD \\
\midrule
None & 39.07 & 25.51 & 45.51 & 31.19 & 55.07 & 39.59 & 66.51 & 43.72 & 50.80 & 39.94 \\
\methodname{} (T5-large) & \textbf{48.60} & \textbf{27.99} & \textbf{54.77} & \textbf{37.21} & \textbf{60.36} & \textbf{41.53} & \textbf{67.85} & \textbf{45.45} & \textbf{59.86} & \textbf{41.90} \\
\quad $\Delta$ & \;+9.53 & \;+2.48 & \;+9.26 & \;+6.02 & \;+5.29 & \;+1.94 & \;+1.34 & \;+1.73 & \;+9.06 & \;+1.96 \\
\midrule
Few-shot GPT-3 (13B) & 46.88 & 28.68 & 52.80 & 43.17 & 59.54 & 45.00 & 67.42 & 52.23 & -- & -- \\
\bottomrule
\end{tabular}
}%
\vspace{-6pt}
\caption{
    Effectiveness of generated knowledge on different QA models.
    Average accuracy on dev set is reported.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_qa}
\vspace{-8pt}
\end{table*}

==> floats/trash/results_ood.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{0.8 \textwidth}{!}{%
\begin{tabular}{l cccccccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multirow{2}{*}{NumerSense} & \multirow{2}{*}{RiddleSense} & \multirow{2}{*}{QuaRTz} & \multirow{2}{*}{HellaSwag} & \multirow{2}{*}{\textbf{Avg.}} \\
\textbf{Knowledge Gen.} $\downarrow$ \\
\midrule
None & 26.50 & 28.11 & 68.75 & 35.00 & 39.59 \\
\methodname{} (T5-large) & \textbf{30.00} & \textbf{30.07} & \textbf{70.31} & \textbf{35.73} & \textbf{41.53} \\
\bottomrule
\end{tabular}
}%
\vspace{2pt}
\caption{
    Results on out-of-domain datasets.
    Accuracy on dev set is reported.
    Predictions made by UnifiedQA-large.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_ood}
\end{table*}

==> floats/trash/results_qa.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{0.66 \textwidth}{!}{%
\begin{tabular}{l cccccccccc}
\toprule
\textbf{QA Model} $\rightarrow$ & \multicolumn{2}{c}{UQA-small} & \multicolumn{2}{c}{UQA-base} & \multicolumn{2}{c}{UQA-large} & \multicolumn{2}{c}{UQA-3b} \\
\textbf{Knowledge Gen.} $\downarrow$ & ID & OOD & ID & OOD & ID & OOD & ID & OOD \\
\midrule
None & 39.07 & 25.51 & 45.51 & 31.19 & 55.07 & 39.59 & 66.51 & 43.72 \\
\methodname{} (T5-large) & \textbf{48.60} & \textbf{27.99} & \textbf{54.77} & \textbf{37.21} & \textbf{60.36} & \textbf{41.53} & \textbf{67.85} & \textbf{45.45} \\
\midrule
$\Delta$ & +9.53 & +2.48 & +9.26 & +6.02 & +5.29 & +1.94 & +1.34 & +1.73 \\
\bottomrule
\end{tabular}
}%
\vspace{-4pt}
\caption{
    Effectiveness of generated knowledge on different QA models.
    Average accuracy on dev set is reported.
    % \textcolor{red}{This is based on \methodname{} trained with reward shape 4, ckpt 5k.}
}
\label{tab:results_qa}
\end{table*}

==> floats/uniknower.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/uniknower.png}
\caption{
    \gary{TODO: Redo this figure.}
    \methodname{} can generate relevant knowledge that grounds the reasoning process for commonsense questions in a wide range of domains.
}
\label{fig:uniknower}
\vspace{-16pt}
\end{figure}
